Multi-Scale Representation Learning for Spatial Feature Distributions using Grid Cells

Unsupervised text encoding models have recently fueled substantial progress in NLP. The key idea is to use neural networks to convert words in texts to vector space representations based on word positions in a sentence and their contexts, which are suitable for end-to-end training of downstream tasks. We see a strikingly similar situation in spatial analysis, which focuses on incorporating both absolute positions and spatial contexts of geographic objects such as POIs into models. A general-purpose representation model for space is valuable for a multitude of tasks. However, no such general model exists to date beyond simply applying discretization or feed-forward nets to coordinates, and little effort has been put into jointly modeling distributions with vastly different characteristics, which commonly emerges from GIS data. Meanwhile, Nobel Prize-winning Neuroscience research shows that grid cells in mammals provide a multi-scale periodic representation that functions as a metric for location encoding and is critical for recognizing places and for path-integration. Therefore, we propose a representation learning model called Space2Vec to encode the absolute positions and spatial relationships of places. We conduct experiments on two real-world geographic data for two different tasks: 1) predicting types of POIs given their positions and context, 2) image classification leveraging their geo-locations. Results show that because of its multi-scale representations, Space2Vec outperforms well-established ML approaches such as RBF kernels, multi-layer feed-forward nets, and tile embedding approaches for location modeling and image classification tasks. Detailed analysis shows that all baselines can at most well handle distribution at one scale but show poor performances in other scales. In contrast, Space2Vec's multi-scale representation can handle distributions at different scales.

==> Location Encoding Paper - ICLR 2020/conclusion.tex <==
\vsection{Conclusion}   %\vspace{-1cm}

We introduced an encoder-decoder framework  as a general-purpose representation model for space inspired by biological grid cells'  multi-scale periodic representations.
The model is an inductive learning model and can be trained in an unsupervised manner. 
%We present different ways to encode point locations as multi-scale periodic representations inspired by grid cell research. 
We conduct two experiments on POI type prediction based on 1) POI locations and 2) nearby POIs. The evaluation results demonstrate the effectiveness of our model. 
%We also visualize the space encoding layer to better showcase the reason why our models perform so well. The visualization indicates that the different neurons of the space encoding layer fire at different locations as place cells do. In fact, their firing patterns reflect the underlying urban structure. 
%\mai{
Our analysis reveals that it is the ability to integrate representations of different scales that makes the grid cell models outperform other baselines on these two tasks.
%}
In the future, we hope to incorporate the presented framework to more complex GIS tasks %to test its generalizability 
% \mai{
such as social network analysis, and sea surface temperature prediction.
%} 
%Moreover, we want to explore the way to encode the locations of places on the surface of the earth directly.



==> Location Encoding Paper - ICLR 2020/context_result.tex <==

% \begin{table}[]
% 	\caption{The evaluation results of different spatial context models on the validation and test dataset.}
% 	\label{tab:conteval}
% 	\centering
% 	\small{ 
% 	\begin{tabular}{c|cccc|ccc}
% 		\toprule
% 		 & \multicolumn{4}{c}{Validation} &    
% 		 \multicolumn{3}{c}{Testing}              \\% \hline
% 		$\modelname$ & MRR            & HIT@1      & HIT@5       & NLL          & MRR            & HIT@1      & HIT@5       \\ \hline
% 		$\model{none}{cont}$         & 0.1579(0.0022) & 6.64(0.24) & 22.37(0.43) & 1.2554(0.0028) & 0.1646(0.0024) & 7.20(0.33) & 22.94(0.40) \\ %\hline
% 		$\model{\naive}{cont}$        & 0.1641(0.0020) & 7.20(0.28) & 23.01(0.46) & 1.2492(0.0032) & 0.1701(0.0024) & 7.62(0.30) & 23.55(0.47) \\ %\hline
% 		$\model{polar}{cont}$        & 0.1694(0.0017) & 7.84(0.20) & 23.65(0.27) & 1.2375(0.0051) & 0.1748(0.0022) & 8.19(0.22) & 24.30(0.39) \\ %\hline
% 		$\model{grid}{cont}$     & 0.1708(0.0021) & 7.68(0.27) & 23.67(0.44) & 1.2354(0.0051) & 0.1820(0.0015) & 8.60(0.16) & 25.35(0.34) \\ %\hline
% 		$\model{hexa}{cont}$ & 0.1720(0.0018) & 7.89(0.20) & 23.70(0.45) & 1.2345(0.0037) & 0.1835(0.0019) & 8.72(0.26) & 25.91(0.36) \\ %\hline
% 		$\model{theorydiag}{cont}$   & 0.1683(0.0030) & 7.47(0.27) & 23.59(0.52) & 1.2448(0.0033) & 0.1738(0.0040) & 7.88(0.44) & 24.40(0.49) \\ %\hline
% 		$\model{theory}{cont}$       & 0.1752(0.0024) & 8.18(0.31) & 24.13(0.41) & 1.2326(0.0048) & 0.1821(0.0023) & 8.61(0.24) & 25.44(0.48) \\ \bottomrule
% 	\end{tabular} }
% \end{table}

% \begin{table}[]
% 	\caption{The evaluation results of different spatial context models on the validation and test dataset.}
% 	\label{tab:conteval_old}
% 	\centering
% 	\small{ 
% 	\begin{tabular}{c|ccc|cc}
% 		\toprule
% 		 & \multicolumn{3}{c}{Validation} &    
% 		 \multicolumn{2}{c}{Testing}              \\% \hline
% 		$\modelname$ & MRR  & HIT@5 & NLL   & MRR     & HIT@5       \\ \hline
% 		$\model{none}{cont}$         
% 		& 0.158 (0.002) &  22.4 (0.4) & 1.255 (0.003) 
% 		& 0.165 (0.002) & 22.9 (0.4) \\ %\hline
% 		$\model{\naive}{cont}$        
% 		& 0.164 (0.002) &  23.0 (0.5) & 1.249 (0.003) 
% 		& 0.170 (0.002) &  23.5 (0.5) \\ %\hline
% 		$\model{polar}{cont}$        
% 		& 0.169 (0.002) &  23.6 (0.3) & 1.237 (0.005) 
% 		& 0.175 (0.002) & 24.3 (0.4) \\ \hline
% 		$\model{rbf}{cont}$  
% 		& 0.170 (0.002) &  23.7 (0.3) & 1.235 (0.005) 
% 		& 0.177 (0.002) & 24.1 (0.4) \\ %\hline
% 		$\model{grid}{cont}$     
% 		& 0.171 (0.002) &  23.7 (0.4) & 1.235 (0.005) 
% 		& 0.182 (0.001) &  25.4 (0.3) \\ %\hline
% 		$\model{hexa}{cont}$ 
% 		& 0.172 (0.002) &  23.7 (0.4) & 1.234 (0.004) 
% 		& 0.184 (0.002) &  25.9 (0.4) \\ %\hline
% 		$\model{theorydiag}{cont}$   
% 		& 0.168 (0.003) &  23.6 (0.5) & 1.244 (0.003) 
% 		& 0.174 (0.004) &  24.4 (0.5) \\ %\hline
% 		$\model{theory}{cont}$       
% 		& 0.175 (0.002) & 24.1 (0.4) & 1.232 (0.005) 
% 		& 0.182 (0.002) &  25.4 (0.5) \\ \hline
% 		$16\_10k\_50\_1h512e64$       
% 		& 0.167 (0.002) & 23.9 (0.4) & 1.230 (0.000) 
% 		& 0.185 (0.002) &  25.4 (0.5) \\
% 		\bottomrule
% 	\end{tabular} }	%\vspace*{-0.55cm}
% \end{table}

\begin{table}[b!]
	\caption{The evaluation results of different spatial context models on the validation and test dataset. %(Place2Vec\_center dataset).
	All encoders contains a 1 hidden layer FFN.
	All grid cell encoders set $\lambda_{min}$=10, $\lambda_{max}$=10k.
	%$\model{scaled\_rbf}{cont}$ set  $\sigma$=40, $\beta$=0.1.
	%\nilao{need std for statistical significance} 
	}
	\label{tab:conteval}
	\centering
	\small{ 
	\begin{tabular}{c|c|ccc|cc}
		\toprule
		 & Train & \multicolumn{3}{c}{Validation} &    
		 \multicolumn{2}{c}{Testing}              \\% \hline
		$\modelname$ & NLL & NLL  & MRR & HIT@5   & MRR     & HIT@5       \\ \hline
		$\model{none}{cont}$         
		& 1.163 & 1.297 & 0.159 (0.002) & 22.4 (0.5) 
		& 0.167 (0.006) & 23.4 (0.7) \\ %\hline
		$\model{\naive}{cont}$ %\cite{chu2019geo}%\_1h512e64$        
		& 1.151 & 1.282  & 0.170 (0.002) & 24.6 (0.4) 
		&  0.175 (0.003) & 24.7 (0.5) \\ %\hline
% 		$\model{\naive}{cont}\_2h512e64$        
% 		& 1.161 & 1.292 & 0.170 (0.0) & 24.6 (0.000) 
% 		&  0.176 (0.000) & 24.9 (0.0) \\ %\hline
% 		$\model{\naive}{cont}\_3h512e64$ 
% 	    %$\model{\naive}{cont}$
% 		& 1.163 & 1.283 & 0.172 (0.0) & 24.2 (0.000) 
% 		&  0.177 (0.000) & 24.0 (0.0) \\ %\hline
        
		$\model{polar}{cont}$%\_1h512e64$        
		& 1.157 & 1.283 & 0.176 (0.004) & 25.4 (0.4) 
		& 0.178 (0.006) & 24.9 (0.1) \\ %\hline
		%\\ \hline
% 		$\model{grid\_tile}{cont} ($c$=200)$        
% 		& 1.162 & 1.287  & 0.157 (0.0) & 22.2 (0.000) 
% 		&  0.171 (0.000) & 23.4 (0.0) \\ %\hline
% 		$\model{grid\_tile}{cont} ($c$=100)$        
% 		& 1.155 & 1.295  & 0.159 (0.0) & 22.9 (0.000) 
% 		&  0.169 (0.000) & 23.4 (0.0) \\ %\hline
		$\model{tile}{cont}$
		%\cite{berg2014birdsnap,adams2015frankenplace,tang2015improving}
		$(c=50)$        
		& 1.163 & 1.298  & 0.173 (0.004) & 24.0 (0.6) 
		&  0.173 (0.001) & 23.4 (0.1) \\ %\hline
% 		$\model{grid\_tile}{cont} ($c$=10)$        
% 		& 1.154 & 1.298  & 0.163 (0.0) & 23.1 (0.000) 
% 		&  0.169 (0.000) & 22.9 (0.0) \\ \hline
        

		

% 		$\model{polar\_tile}{cont} ($\freq$=16)$        
% 		& 1.147 & 1.287  & 0.167 (0.0) & 23.6 (0.000) 
% 		&  0.163 (0.000) & 22.3 (0.0) \\ %\hline
		$\model{polar\_tile}{cont} (\freq=64)$        
		& 1.161 & 1.282  & 0.173 (0.003) & 25.0 (0.1) 
		&  0.177 (0.001) & 24.5 (0.3) \\ % \hline

%         Mac Aodha et al. \cite{mac2019presence} ($1h64e64_n$)   
% 		& 1.167 & 1.297  & 0.162 (0.004) & 23.1 (0.6) 
% 		&  0.162 (0.000) & 22.9 (0.0) \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($1h512e64$)      
% 		& 1.162 & 1.291  & 0.160 (0.004) & 22.9 (0.6) 
% 		&  0.170 (0.000) & 23.8 (0.0) \\ %\hline
		$\model{\aodha}{cont}$ 
		%\cite{mac2019presence} 
		($\numresnet$=2,$\numneuron$=512)      
		& 1.167 & 1.291  & 0.159 (0.001) & 23.0 (0.1) 
		&  0.170 (0.001) & 23.9 (0.2) \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($3h512e64$) 
% 		& 1.176 & 1.289  & 0.159 (0.004) & 22.6 (0.6) 
% 		&  0.167 (0.000) & 23.3 (0.0) \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($4h512e64$) 
% 		& 1.168 & 1.293  & 0.165 (0.004) & 23.0 (0.6) 
% 		&  0.168 (0.000) & 23.5 (0.0) \\ %\hline


% 		$\model{rbf}{cont}\_n100\_500\_0.0\_1h512e64$  
% 		& 1.176 & 1.300 & 0.156 (0.0) & 22.1 (0.000) 
% 		& 0.166 (0.000) &  23.4 (0.0) \\ %\hline
% 		$\model{rbf}{cont}\_n100\_200\_0.0\_1h512e64$  
% 		& 1.163 & 1.286 & 0.165 (0.0) & 22.9 (0.000) 
% 		& 0.166 (0.000) &  23.9 (0.0) \\ %\hline
% 		$\model{rbf}{cont}\_n100\_100\_0.0\_1h512e64$  
% 		&  1.162 & 1.292 & 0.170 (0.0) & 24.5 (0.000) 
% 		&  0.173 (0.000) &  24.9 (0.0) \\ %\hline
		$\model{rbf}{cont}$ $(\sigma=50)$%\_n100\_50\_0.0\_1h512e64$  
		&  1.160 & 1.281  & \textbf{0.179} (0.002) & 25.2 (0.6) 
		&  0.172 (0.001) &  25.0 (0.1) \\ %\hline
% 		$\model{rbf}{cont}\_n100\_10\_0.0\_1h512e64$  
% 		&  1.152 & 1.278 & 0.176 (0.0) & 24.4 (0.000) 
% 		&  0.174 (0.000) &  24.4 (0.0) \\ %\hline
% 		$\model{rbf}{cont}\_n100\_5\_0.0\_1h512e64$  
% 		&  1.154 & 1.274 & 0.175 (0.0) & 24.2 (0.000) 
% 		&  0.174 (0.000) &  24.1 (0.0) \\ \hline
		
% 		$\model{rbf}{cont}\_n100\_10\_0.1\_1h512e64$  
% 		&  1.168 & 1.290 & 0.172 (0.0) & 24.5 (0.000) 
% 		&  0.181 (0.000) &  25.2 (0.0) \\ %\hline
% 		$\model{rbf}{cont}\_n100\_20\_0.1\_1h512e64$  
% 		&  1.157 & 1.287 & 0.174 (0.0) & 24.6 (0.000) 
% 		&  0.182 (0.000) &  25.2 (0.0) \\ %\hline
		$\model{scaled\_rbf}{cont}$ ($\sigma$=40,$\beta$=0.1) %(\sigma=40,\beta=0.1)$%\_n100\_40\_0.1\_1h512e64$  
		&  1.150 & 1.272 & 0.177 (0.002) & \textbf{25.7} (0.1) 
		&  0.181 (0.001) &  25.3 (0.1) \\ %\hline
% 		$\model{rbf}{cont}\_n100\_10\_0.2\_1h512e64$  
% 		&  1.172 & 1.289  & 0.171 (0.0) & 23.2 (0.000) 
% 		&  0.178 (0.000) &  25.4 (0.0) \\ %\hline
% 		$\model{rbf}{cont}\_n100\_10\_0.3\_1h512e64$  
% 		&  1.152 & 1.276  & 0.178 (0.0) & 25.1 (0.000) 
% 		&  0.182 (0.000) &  24.4 (0.0) \\ %\hline
% 		$\model{rbf}{cont}\_n100\_10\_0.4\_1h512e64$  
% 		&  1.164 & 1.285 & 0.175 (0.0) & 23.8 (0.000) 
% 		&  0.178 (0.000) &  24.8 (0.0) \\ 
\hline

		$\model{grid}{cont}$($\lambda_{min}$=10)%\_16\_10k\_10\_1h512e64$     
		& 1.172 & 1.285 & 0.178 (0.004) & 24.9 (0.5) 
		& 0.181 (0.001) & 25.1 (0.3) \\ %\hline
% 		$\model{grid}{cont}\_16\_10k\_5\_1h512e64$     
% 		& 1.160 & 1.273 & 0.176 (0.0) & 25.0 (0.000) 
% 		& 0.181 (0.000) & 25.3 (0.0) \\ %\hline
		$\model{hexa}{cont}$ ($\lambda_{min}$=10)
		& 1.156 & 1.289  & 0.173 (0.002) & 24.0 (0.2) 
		& 0.183 (0.002) & 25.3 (0.2) \\ %\hline
		$\model{theorydiag}{cont}$ $(\lambda_{min}=10)$% \_16\_10k\_10\_1h512e64$   
		& 1.156 & 1.287 &  0.168 (0.001) & 24.1 (0.4) 
		& 0.174 (0.005) & 24.9 (0.1) \\ %\hline
% 		$\model{theory}{cont}$       
% 		&   &  &  (0.0) &  (0.000) 
% 		&  (0.000) &   (0.0) \\ %\hline
% 		$\model{theory}{cont}\_16\_10k\_50\_1h512e64$       
% 		& 1.171 & 1.290 & 0.176 (0.000) & 24.1 (0.0) 
% 		& 0.178 (0.000) &  25.0 (0.0) \\
% 		$\model{theory}{cont}\_16\_10k\_10\_1h512e64$       
% 		& 1.170 & 1.288  & 0.180 (0.000) & 35.0 (0.0) 
% 		& 0.181 (0.000) &  25.5 (0.0) \\
% 		$\model{theory}{cont}\_16\_10k\_5\_1h512e64$       
% 		& 1.164 & 1.278 & 0.175 (0.000) & 25.0 (0.0) 
% 		& 0.180 (0.000) &  25.3 (0.0) \\
% 		$\model{theory}{cont}\_64\_10k\_200\_1h512e64$       
% 		& 1.158 & 1.295 & 0.159 (0.000) & 23.1 (0.0) 
% 		& 0.170 (0.000) &  23.0 (0.0) \\
% 		$\model{theory}{cont}\_64\_10k\_100\_1h512e64$       
% 		& 1.158 & 1.290 & 0.169 (0.000) & 24.3 (0.0) 
% 		& 0.176 (0.000) &  24.3 (0.0) \\
% 		$\model{theory}{cont}\_64\_10k\_50\_1h512e64$       
% 		& 1.158 & 1.275 & 0.171 (0.000) & 23.9 (0.0) 
% 		& 0.173 (0.000) &  24.8 (0.0) \\
		$\model{theory}{cont}$($\lambda_{min}$=200)%\_64\_10k\_200\_1h512e64$       
		& 1.168 & 1.295 & 0.159 (0.001) & 23.1 (0.2) 
		& 0.170 (0.001) &  23.2 (0.2) \\
% 		$\model{theory}{cont}$($\lambda_{min}$=100)%\_64\_10k\_100\_1h512e64$       
% 		& 1.152 & 1.290 & 0.169 (0.003) & 24.3 (0.3) 
% 		& 0.176 (0.003) &  24.3 (0.4) \\
		$\model{theory}{cont}$($\lambda_{min}$=50)%\_64\_10k\_50\_1h512e64$       
		& 1.157 & 1.275 & 0.171 (0.001) & 24.2 (0.3) 
		& 0.173 (0.001) &  24.8 (0.4) \\
		$\model{theory}{cont}$($\lambda_{min}$=10)%\_64\_10k\_10\_1h512e64$       
		& 1.158 & 1.280 & 0.177 (0.003) & 25.2 (0.3) 
		& \textbf{0.185} (0.002) &  \textbf{25.7} (0.3) \\
% 		$\model{theory}{cont}$%(\lambda_{min}=10)$%\_64\_10k\_10\_1h512e64$       
% 		& 1.153 & 1.275 & 0.180 (0.000) & 25.2 (0.0) 
% 		& 0.177 (0.000) &  24.4 (0.0) \\
%       $\model{theory}{cont}\_64\_10k\_10\_1h512e64$       
% 		& 1.158 & 1.280 & 0.173 (0.000) & 24.3 (0.0) 
% 		& 0.185 (0.002) &  25.7 (0.006) \\
% 		$\model{theory}{cont}\_64\_10k\_10\_2h512e64$       
% 		& 1.156 & 1.280 & 0.177 (0.000) & 25.1 (0.0) 
% 		& 0.184 (0.000) &  25.2 (0.0) \\
% 		$\model{theory}{cont}\_64\_10k\_10\_3h512e64$       
% 		& 1.155 & 1.285 & 0.176 (0.000) & 25.2 (0.0) 
% 		& 0.180 (0.000) &  24.9 (0.0) \\
		\bottomrule
	\end{tabular} }	%\vspace*{-0.55cm}
\end{table}




==> Location Encoding Paper - ICLR 2020/context_viz.tex <==
%\subsection{Context Modeling Visualizations} \label{sec:apdx:context}


Figure~\ref{fig:poicl} shows the location embedding clustering results in both 
Cartesian and polar  coordinate systems.
% Similar hierarchical clustering is performed on the location embeddings produced by the space encoders of different models. Fig. \ref{fig:cont_naive}, \ref{fig:cont_polar}, \ref{fig:cont_aodha}, \ref{fig:cont_polar_tile}, \ref{fig:cont_rbf_01_}, \ref{fig:cont_theory_10_} show the clustering results of $\model{\naive}{cont}$, $\model{polar}{cont}$, $\model{\aodha}{cont}$ \citep{mac2019presence} ($\numresnet=2,\numneuron=512$), $\model{polar\_tile}{cont}$, $\model{scaled\_rbf}{cont}$ ($\sigma=40,\beta=0.1$), and $\model{theory}{cont}$ ($\lambda_{min}=10$) on the relative spatial context $A_{cont}$. Fig. \ref{fig:cont_naive_polar}, \ref{fig:cont_polar_polar},
% \ref{fig:cont_aodha_polar}, \ref{fig:cont_polar_tile_polar}, \ref{fig:cont_rbf_01_polar_}, \ref{fig:cont_theory_10_polar_} shows the clustering results of the corresponding models in the polar coordinate system $(r, \theta)$ where $r = log(\Delta\bx_{ij} + 1)$. 
We can see that  $\model{\naive}{cont}$ (Fig. \ref{fig:cont_naive}, \ref{fig:cont_naive_polar}) only captures  the distance information when the context POI is very  close ($log(\parallel\Delta\bx_{ij}\parallel + 1) \leq 5$) while in the farther spatial context it purely models the direction information. 
$\model{polar}{cont}$ (Fig. \ref{fig:cont_polar}, \ref{fig:cont_polar_polar}) has the similar behaviors but captures the distance information in a more fine-grained manner. 
$\model{\aodha}{cont}$ (Fig. \ref{fig:cont_aodha}, \ref{fig:cont_aodha_polar}) mainly focuses on differentiating relative positions in farther spatial context $\cont$ which might explain its lower performance\footnote{Note that $\model{\aodha}{cont}$ is original proposed by \citet{mac2019presence} for location modelling, not spatial context modelling. This results indicates $\model{\aodha}{cont}$  is not good at this task.}.
$\model{polar\_tile}{cont}$ (Fig. \ref{fig:cont_polar_tile})
%the pattern is not very clear but it 
mostly responds to distance information. 
Interestingly, $\model{scaled\_rbf}{cont}$ and $\model{theory}{cont}$  have similar representations in the polar coordinate system (Fig. \ref{fig:cont_rbf_01_polar_}, \ref{fig:cont_theory_10_polar_}) and similar performance (Table \ref{tab:conteval}). 
% This indicates that they capture similar information. 
While $\model{scaled\_rbf}{cont}$  captures the gradually decreased distance effect with a scaled kernel size which becomes larger in farther distance, $\model{theory}{cont}$ achieves this by integrating representations of different scales. 
%Since $\model{scaled\_rbf}{cont}$ has to remember all anchor point information during testing time, we still champion the grid cell model in the spatial context modeling.

%In fact, $\model{polar}{cont}$ shows a competitive performance. One explanation is that the most important feature the spatial relationship embeddings capture is the distance between the center point and context points. By converting $\Delta\bx_{ij}$ into polar coordinates, the distance feature is explicitly feet into the model which boost the model performance.




% \begin{figure*}[h!]
% 	%\vspace*{-0.35cm}
% 	\centering
% 	\begin{subfigure}[b]{0.28\textwidth} 
% 		\centering 
% 		\includegraphics[width=\textwidth]{./fig/relative_naive_cluster_10_new.png}
% 		%\vspace{-0.15cm}
% 		\caption{}
% 		\label{fig:contnaivecluster}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.28\textwidth} 
% 		\centering 
% 		\includegraphics[width=\textwidth]{./fig/relative_polar_cluster_10_new.png}
% 		%\vspace{-0.15cm}
% 		\caption{}
% 		\label{fig:contpolarcluster}
% 	\end{subfigure}
% 	%\hfill
% 	\begin{subfigure}[b]{0.28\textwidth}  
% 		\centering 
% 		\includegraphics[width=\textwidth]{./fig/relative_theory_cluster_10_new.png}
% 		%\vspace{-0.15cm}
% 		\caption{}
% 		\label{fig:conttheorycluster}
% 	\end{subfigure}
% 	\vspace*{-0.25cm}
% 	\caption{The Hierarchical clustering results of the location embeddings from the spatial context model $\model{naive}{cont}$ (a),  $\model{polar}{cont}$ (b), and $\model{theory}{cont}$ (c). The scale is in meters.
% 	%\nilao{increase resolution, and use none-gradient legend as in Fig 1}
% 	} 
% 	\label{fig:contcluster}
% 	\vspace*{-0.05cm}
% \end{figure*}

%We also visualize the clustering results of the result location embeddings of $\model{\naive}{cont}$, $\model{polar}{cont}$, and $\model{theory}{cont}$ as shown in Fig. \ref{fig:contnaivecluster}, \ref{fig:contpolarcluster}, and \ref{fig:conttheorycluster}. Most information capture by the space encoder of $\model{\naive}{cont}$ is  direction information while $\model{theory}{cont}$ captures  distance information; see appendix for all the response maps.


\begin{figure*}[t!]
	\centering \tiny
	\vspace*{-0.2cm}
	\begin{subfigure}[b]{0.16\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/cont_naive_1h512e64.png}\vspace*{-0.2cm}
		\caption[]%
		{{\small 
		%$%\model{rbf}{loc} 
		$\model{\naive}{cont}$
		}}    
		\label{fig:cont_naive}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.165\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/cont_polar_1h512e64.png}\vspace*{-0.1cm}
		\caption[]%
		{{\small 
		%$%\model{rbf}{loc} 
		$\model{polar}{cont}$
		}}    
		\label{fig:cont_polar}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.16\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/cont_aodha_2h512e64_none.png}\vspace*{-0.2cm}
		\caption[]%
		{{\small 
		%$%\model{rbf}{loc} 
		$\model{\aodha}{cont}$ %($\numresnet$=2,$\numneuron$=512)
		}}    
		\label{fig:cont_aodha}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.16\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/cont_polartile_64_1h512e64.png}\vspace*{-0.15cm}
		\caption[]%
		{{\small  
		%$\model{theory}{loc} 
		$\model{polar\_tile}{cont}$ %($\freq$=64) %, \lambda_{max}=40k$ 
		}}    
		\label{fig:cont_polar_tile}
	\end{subfigure}
	\hfill
    \begin{subfigure}[b]{0.165\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/{cont_rbf_n100_10_0.1_1h512e64}.png}\vspace*{-0.03cm}
		\caption[]%
		{{\small  
		%$\model{theory}{loc} 
		$\model{scaled\_rbf}{cont}$ %($\beta$=0.1) %, \lambda_{max}=40k$ 
		}}    
		\label{fig:cont_rbf_01_}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.16\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/cont_theory_64_10k_10_1h512e64.png}\vspace*{-0.2cm}
		\caption[]%
		{{\small 
		%$\model{theory}{loc}$ 
		$\model{theory}{cont}$ %($\lambda_{min}$=10)%, \lambda_{max}=40k$ 
		}}    
		\label{fig:cont_theory_10_}
	\end{subfigure}
	\begin{subfigure}[b]{0.155\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/cont_naive_1h512e64-polar.png}\vspace*{-0.2cm}
		\caption[]%
		{{\small 
		%$%\model{rbf}{loc} 
		$\model{\naive}{cont}$
		}}    
		\label{fig:cont_naive_polar}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.155\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/cont_polar_1h512e64-polar.png}\vspace*{-0.2cm}
		\caption[]%
		{{\small 
		%$%\model{rbf}{loc} 
		$\model{polar}{cont}$
		}}    
		\label{fig:cont_polar_polar}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.16\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/cont_aodha_2h512e64_none-polar.png}\vspace*{-0.2cm}
		\caption[]%
		{{\small 
		%$%\model{rbf}{loc} 
		$\model{\aodha}{cont}$ %($\numresnet$=2,$\numneuron$=512)
		}}    
		\label{fig:cont_aodha_polar}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.16\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/cont_polartile_64_1h512e64-polar.png}\vspace*{-0.2cm}
		\caption[]%
		{{\small  
		%$\model{theory}{loc} 
		$\model{polar\_tile}{cont}$ %($\freq$=64) %, \lambda_{max}=40k$ 
		}}    
		\label{fig:cont_polar_tile_polar}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.145\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/{cont_rbf_n100_10_0.1_1h512e64-polar}.png}\vspace*{-0.1cm}
		\caption[]%
		{{\small  
		%$\model{theory}{loc} 
		$\model{scaled\_rbf}{cont}$ %($\beta$=0.1) %, \lambda_{max}=40k$ 
		}}    
		\label{fig:cont_rbf_01_polar_}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.16\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/cont_theory_64_10k_10_1h512e64-polar.png}\vspace*{-0.2cm}
		\caption[]%
		{{\small 
		%$\model{theory}{loc}$ 
		$\model{theory}{cont}$ %($\lambda_{min}$=10)%, \lambda_{max}=40k$ 
		}}    
		\label{fig:cont_theory_10_polar_}
	\end{subfigure}
	\caption{%Compare 
	%\small
	Embedding clustering in the original space of 
	(a) $\model{\naive}{cont}$; 
	(b) $\model{polar}{cont}$; 
	(c) $\model{\aodha}{cont}$, $\numresnet$=2,$\numneuron$=512; 
	(d) $\model{polar\_tile}{cont}$, $\freq$ = 64, 
	(e) $\model{scaled\_rbf}{cont}$, $\sigma$ = 40, $\beta$=0.1; and
	(f) $\model{theory}{cont}$, $\lambda_{min}=10$, $\lambda_{max}=10k$, $\nscale = 64$. 
	(g)(h)(i)(j)(k)(l) are the  clustering results of the same models in the polar-distance space using $\log(\parallel\Delta\bx_{ij}\parallel + 1)$. All models use 1 hidden ReLU (except $\model{\aodha}{cont}$) layers of 512 neurons. %FFN.
	Most models except  $\model{\aodha}{cont}$ can capture a shift when distance is around $e^5-1 \approx 150$ meters.
	} 
	\label{fig:poicl}
	\vspace*{-0.15cm}
\end{figure*}

==> Location Encoding Paper - ICLR 2020/decoder.tex <==
\vspace{-0.5cm}
\vsubsection{Decoder}   \label{sec:dec} 
Two types of decoders are designed for two major types of GIS problems: location modeling and spatial context modeling (See Section \ref{sec:dataset}).
\paragraph{Location Decoder}            \label{sec:locdec}
 $\locdec()$ directly reconstructs point feature embedding $\feemb{i}$ given its space embedding $\peemb{i}$. We use one layer feed-forward neural network $\locdecmlp()$ %to do this (See Equ. \ref{equ:decloc}). 
\begin{align}
\feemb{i}^{\prime} = \locdec( \bx_i; \locdectheta) = \locdecmlp(\peemb{i})
\label{equ:decloc}
\end{align}
For training we use inner product to compare the reconstructed feature embedding $\feemb{i}^{\prime}$ against the real feature embeddings of $\feemb{i}$ and other negative points (see training detail in Sec~\ref{sec:training}).

\paragraph{Spatial Context Decoder}       \label{sec:contdec}
$\contdec()$ reconstructs the feature embedding $\feemb{i}$ of the center point $p_i$ based on the space and feature embeddings $\{\emb_{i1},...,\emb_{ij},...,\emb_{i\neisize}\}$ of $\neisize$ nearby points $\{p_{i1},...,p_{ij},...,p_{i\neisize}\}$. 
Note that the feed-in order of context points %embeddings feed-in 
 should not affect the prediction results, which can be achieved by 
 %. In other words, we need a 
permutation invariant neural network architectures \citep{zaheer2017deep} like PointNet \citep{qi2017pointnet}. 
%We can compute the feature embedding of a point with a multi-head attention  by using the embeddings of $\neisize$ context points.
\begin{align}
\feemb{i}^{\prime} = \contdec(\bx_i,
\{\emb_{i1},...,\emb_{ij},...,\emb_{i\neisize}\} ; \contdectheta) 
= \attnact(\dfrac{1}{\attnsize} \sum_{\attnidx=1}^{\attnsize} \sum_{j=1}^{\neisize} \attnscr_{ij\attnidx}\feemb{ij}) 
\label{equ:dec_gc}
\end{align}
Here $\attnact$ is an activation function such as sigmoid. $\attnscr_{ij\attnidx}=  \frac{exp(\sigma_{ijk})}{\sum_{o=1}^{\neisize} exp(\sigma_{iok})}$ is the attention of $p_{i}$
%the $i$th example 
with its $j$th neighbor through the $k$th attention head, and 
%\nlao{we might want to experiment with a more complex MLP here to learn spatial relation representation.}
%\nlao{we might also compare $\peemb{i}-\peemb{ij}$ vs $\peemb{i}+\peemb{ij}$ vs $\mathbf{e}[\bx_{i}-\bx_{ij}]$}
\begin{align}
%\attnscr_{ij\attnidx}
%= \attnfun_{\attnidx}(\spemb_{i}, \spemb_{ij})
% = \dfrac{exp(\sigma_{i,j})}{\sum_{o=1}^{\neisize} exp(\sigma_{i,o})} \\
\sigma_{ijk} = \leakyrelu(\attnvec_k^{T}[\feemb{i}_{init}; \feemb{ij};\mathbf{e}[\bx_{i}-\bx_{ij}] ])
\label{equ:atten_gc}
\end{align}
%Equation \ref{equ:atten_gc} shows how to use the attention mechanism to compute the attention score for each nearby point $p_{ij}$. 
where $\attnvec_{\attnidx} \in \Real^{2\fedim+\pedim}$ is the attention parameter in the $\attnidx$th attention head. 
%$[;]$ represents vector concatenation operation. 
The multi-head attention mechanism is inspired by Graph Attention Network \citep{velivckovic2017graph} and \citet{mai2019contextual}. 

To represent the spatial relationship (distance and direction) %distance 
between each context point $p_{ij} = (\bx_{ij}, \bv_{ij})$ and the center point $p_i = (\bx_i, \bv_i)$,
%as well as the direction relationship in the center point embedding reconstruction process, 
we use the space encoder $\enc^{(x)}()$ to encode the displacement between them $\Delta\bx_{ij} = \bx_{i}-\bx_{ij}$. 
Note that we are 
%not focusing on modeling the pairwise spatial interactions between center point and one context point but on 
modeling the spatial interactions between the center point and  $\neisize$ context points simultaneously. 
%As far as we know, this is the first neural network model to do so for point datasets. 

In Eq. \ref{equ:atten_gc}, $\feemb{i}_{init}$ indicates the initial guess of the feature embedding $\feemb{i}$ of point $p_i$ which is computed by using another multi-head attention layer as Eq. \ref{equ:dec_gc} where the weight $\attnscr_{ij\attnidx}^{\prime}=  \frac{exp(\sigma_{ijk}^{\prime})}{\sum_{o=1}^{\neisize} exp(\sigma_{iok}^{\prime})}$. Here, $\sigma_{ijk}^{\prime}$ is computed as Eq. \ref{equ:atten_init} where the query embedding $\feemb{i}$ is excluded.

\vspace{-0.4cm}
\begin{align}
	\sigma_{ijk}^{\prime} = \leakyrelu(\attnvec_{k}^{\prime T}[ \feemb{ij};\mathbf{e}[\bx_{i}-\bx_{ij}] ])
	\label{equ:atten_init}
\end{align}





==> Location Encoding Paper - ICLR 2020/defs.tex <==
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{mathabx}
\usepackage{xspace}
% \usepackage{amssymb}
\usepackage{color}
\usepackage{pgfplots, pgfplotstable}
\usepackage[colorinlistoftodos]{todonotes} %todo

\newcommand{\mn}[1]{\textcolor{blue}{{(MN: #1)}}}
\newcommand{\nlao}[1]{\textcolor{purple}{{(NL: #1)}}}
\newcommand{\cl}[1]{\textcolor{red}{{(CL: #1)}}}
\newcommand{\jb}[1]{\textcolor{brown}{{(JB: #1)}}}
%\newcommand{\todo}[1]{\textcolor{orange}{(TODO: #1)}}
\newcommand{\comment}[1]{}

%\newcommand{\argmax}[1]{\underset{#1}{\operatorname{argmax}}}
% \newcommand{\argmax}{\operatornamewithlimits{argmax}}
% \newcommand{\argmin}[1]{\underset{#1}{\operatorname{argmin}}}
\newcommand{\logsumexp}[0]{\mathrm lse}
\def\etal{{\em et al.\xspace}}

\def\nsm{Neural Semantic Machine\xspace}
\def\NSM{NSM\xspace}

\def\mapo{Memory Augmented Policy Optimization\xspace}
\def\MAPO{MAPO\xspace}
\def\EMAPO{EMAPO\xspace}

\def\npp{Neural Program Planner\xspace}
\def\NPP{NPP\xspace}
%$\theta_{np}$ 

\def\pprob{p^\mathrm{prob}}
\def\pp{p^\mathrm{prob}}
\def\tprob{t^\mathrm{prob}} 
\def\tp{t^\mathrm{prob}} 
\def\qtitle{q^\mathrm{title}}
\def\qcol{q^\mathrm{col}}
\def\qtok{q^\mathrm{tok}}
\def\tagree{t^\mathrm{agree}}
\def\qattn{\vec{q}^\mathrm{attn}}

% \newcommand{\supp}[0]{supp. material}
% \newcommand{\extra}[1]{}
% \newcommand{\extracite}[1]{}
\newcommand{\extra}[1]{#1}
\newcommand{\extracite}[1]{#1}
\newcommand{\supp}[0]{Appendix~\ref{app:rml-proofs}}
\def\REINFORCE{REINFORCE\xspace}

\renewcommand{\vec}[1]{\boldsymbol{\mathbf{#1}}}
\def\btheta{\vec{\theta}}
\def\A{\mathcal{A}}
\def\piB{\pi_\B}
\def\piBo{\pi_\B^{\text{old}}}
\def\B{\mathcal{B}}
\def\Ba{\mathcal{B}_a}
\def\Br{\mathcal{B}_r}
\def\a{a}
\def\r{R}
\def\ba{\vec{a}}
\def\bb{\vec{b}}
\def\bc{\vec{c}}
\def\bd{\vec{d}}
\def\be{\vec{e}}
\def\bbf{\vec{f}} % ugh, oh well
\def\bg{\vec{g}}
\def\bh{\vec{h}}
\def\bi{\vec{i}}
\def\bj{\vec{j}}
\def\bk{\vec{k}}
\def\bl{\vec{l}}
\def\bm{\vec{m}}
\def\bn{\vec{n}}
\def\bo{\vec{o}}
\def\bp{\vec{p}}
\def\bq{\vec{q}}
\def\br{\vec{r}}
\def\bs{\vec{s}}
\def\bt{\vec{t}}
\def\bu{\vec{u}}
\def\bv{\vec{v}}
\def\bw{\vec{w}}
\def\bx{\vec{x}}
\def\by{\vec{y}}
% \nl{let's use z for the programs since they are hidden?} 
% \ml{a stands for action}
\def\ba{\vec{a}}
\def\bas{\vec{a}^*}
\def\bz{\vec{z}}

\def\bxi{\bx^{(i)}}
\def\bysi{\by^{(i)*}}

\def\mF{\mathcal{F}}
\def\mY{\mathcal{Y}}
\def\mX{\mathcal{X}}
\def\mL{\mathcal{L}}
\def\mP{\mathcal{P}}
\def\Real{\mathbb{R}}
\def\Complex{\mathbb{C}}

\def\bC{\mathbf{C}}
\def\bO{\mathbf{O}}
\def\bD{\mathbf{D}}

\def\mLSTM{\mathrm{LSTM}}
\def\mReLU{\mathrm{ReLU}}
\def\mTanh{\mathrm{Tanh}}
\def\mCNN{\mathrm{CNN}}
\def\mLinear{\mathrm{Linear}}

%%% Notation based on Mohammad's preference %%%
%\def\targetr{\tilde{q}}         % target logits
%\def\targetp{q}                 % target prob
%\def\modelr{\tilde{p}_{\theta}} % model logits
%\def\modelp{p_{\theta}}         % model prob
%\def\anyr{\tilde{p}}            % generic logits
%\def\anyp{p}                    % generic prob
%\def\midr{\tilde{m}}            % midpoint logits
%\def\altr{\tilde{a}}            % alternate logits
%\def\altaltr{\tilde{b}}         % alternate2 logits
%\def\domain{\tilde\calF}        % bregman domain
%\def\range{\calF}               % bregman range

%%% Alternative notation based on Dale's preference %%%
% Sorry, I'm not trying to be stubborn!  
% This just seems to make the Bregman section a lot easier to read,
% without harming the readability of the other sections.
\def\targetr{r}               % target logits
\def\targetp{q}               % target prob
\def\modelr{\hat{r}_{\theta}} % model logits
\def\modelp{{p}_{\theta}} % model prob
\def\anyr{{s}}            % generic logits
\def\anyp{{p}}            % generic prob
\def\midr{\smallfrac{q+p}{2}}                  % midpoint logits
\def\altr{a}                  % alternate logits
\def\altaltr{b}               % alternate2 logits
\def\domain{\calF}            % bregman domain
\def\range{\calF^*}           % bregman range
\def\softmax{f^*}

\def\eps{\epsilon}

\def\bys{{\mathbf y}^*}
\def\byp{{\mathbf y}} % \widetilde
\def\byt{\widetilde{\mathbf y}}
\def\temp{\tau}
\def\lossml{\mathcal{L}_{\mathrm{ML}}}
\def\lossrml{\mathcal{L}_{\mathrm{RAML}}}

\def\obj{\mathcal{O}}
\def\objml{\mathcal{O}_{\mathrm{CLL}}}
\def\objmml{\mathcal{O}_{\mathrm{MML}}}
\def\objrml{\mathcal{O}_{\mathrm{RAML}}}
\def\objrl{\mathcal{O}_{\mathrm{RL}}}
\def\objmix{\mathcal{O}_{\mathrm{AUG}}}
%\def\objmix{\mathcal{J}_{\mathrm{mix}}}
\def\lossrl{\mathcal{L}_{\mathrm{RL}}}
\def\objer{\mathcal{O}_{\mathrm{ER}}}
\def\objmapo{\mathcal{O}_{\mathrm{MAPO}}}
\def\objnpp{\mathcal{O}_{\mathrm{NPP}}}

\def\dataset{\mathcal{D}}
\def\klrange{\Delta^{|\calY|}}
\def\diag{\mathrm{Diag}}
\def\int{\mathrm{int}}
% \DeclareMathOperator{\E}{\mathbb{E}}
% \DeclareMathOperator{\Var}{\mathrm{Var}}
% \DeclareMathOperator{\Cov}{\mathrm{Cov}}

\newcommand{\reward}[2]{r(#1, #2)}
\newcommand{\bleu}[2]{\mathrm{BLEU}(#1, #2)}
\newcommand{\simi}[2]{\mathrm{SIM}(#1, #2)}
\newcommand{\kl}[2]{D_{\mathrm{KL}}\left(#1~\Vert~#2\right)}
\newcommand{\dv}[3]{D_{#1}\left(#2~\Vert~#3\right)}
\newcommand{\df}[2]{\dv{F}{#1}{#2}}
\newcommand{\dfs}[2]{\dv{F^*}{#1}{#2}}
\newcommand{\dfst}[2]{\dv{F^*_\temp}{#1}{#2}}
\newcommand{\ent}[1]{\mathbb{H}\left(#1\right)}
\newcommand{\inner}[2]{\langle#1,#2\rangle}

\newcommand{\trans}[1]{{#1}^{\ensuremath{\mathsf{T}}}}

\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}

\def\eg{{\em e.g.}}
\def\ie{{\em i.e.}}
\def\vs{{\em v.s.}\xspace}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newcounter{prop}
\newtheorem{proposition}[prop]{Proposition}
%\newenvironment{proof}{\par\noindent{\em Proof:\ }}{\hfill$\blacksquare$\\}
%\newenvironment{proof}[1]{\par\noindent{\em Proof of #1:\ }}{\hfill$\blacksquare$\\}

\newcommand{\tabref}[1]{Table~\ref{#1}}
% \newcommand{\figref}[1]{Figure~\ref{#1}}
% \newcommand{\secref}[1]{Section~\ref{#1}}


\def\subspace{-0.2cm}
%\def\pit{\pi_\theta}
\def\pip{\pi_\phi}
\def\expected{\mathbb{E}}
\def\oldpi{\pi_\theta^{old}}
\def\buf{\mathcal{B}}

% \algdef{SE}[SUBALG]{Indent}{EndIndent}{}{\algorithmicend\ }%
% \algtext*{Indent}
% \algtext*{EndIndent}

% \newlength\myindent
% \setlength\myindent{2em}
% \newcommand\bindent{%
%     \begingroup
%     \setlength{\itemindent}{\myindent}
%     \addtolength{\algorithmicindent}{\myindent}
% }
% \newcommand\eindent{\endgroup}


\newcommand{\modelname}{Space2Vec }
\newcommand{\model}[2]{{#1}}
%\newcommand{\model}[2]{s2v\_{#2}\_{#1}}

\newcommand{\relu}{ReLU}
\newcommand{\leakyrelu}{LeakyReLU}

\newcommand{\loss}{\mathcal{L}}

\newcommand{\dist}{\mathbf{\Phi}}

\newcommand{\emb}{\mathbf{e}}
\newcommand{\nei}{C}
\newcommand{\neisize}{n}

\newcommand{\spdim}{L}
\newcommand{\nscale}{S}


\newcommand{\pedim}{d^{(x)}}
\newcommand{\fedim}{d^{(v)}}
\newcommand{\embdim}{d}

\newcommand{\peemb}[1]{\mathbf{e}[\bx_{#1}]}
\newcommand{\feemb}[1]{\mathbf{e}[\bv_{#1}]}
% \newcommand{\peemb}{\mathbf{e}_{(x)}}
% \newcommand{\feemb}{\mathbf{e}_{(v)}}

\newcommand{\pose}{PE}

\newcommand{\negsize}{N}
%\newcommand{\negsamp}{Neg}
\newcommand{\negsamp}{\mathcal{N}}
\newcommand{\negsampi}{\negsamp_i}

\newcommand{\attnfun}{\mathbf{A}}
\newcommand{\attnscr}{\alpha}
\newcommand{\attnvec}{\mathbf{a}}
\newcommand{\attnsize}{K}
\newcommand{\attnidx}{k}
\newcommand{\attnact}{g} %\sigma}

\newcommand{\freq}{S}

\newcommand{\enc}{Enc}
\newcommand{\enctheta}{\mathbf{\theta}_{\text{enc}}}

%\newcommand{\vssec}{\vspace{-0.2cm}}
\newcommand{\vsection}[1]{
\vspace{-0.2cm}
\section{#1}
\vspace{-0.2cm}
}
\newcommand{\vsubsection}[1]{
\vspace{-0.2cm}
\subsection{#1}
\vspace{-0.2cm}
}

\newcommand{\vsubsubsection}[1]{
\vspace{-0.05cm}
\subsubsection{#1}
\vspace{-0.1cm}
}

\newcommand{\dec}{Dec}
\newcommand{\dectheta}{\mathbf{\theta}_{\text{dec}}}

\newcommand{\locdec}{Dec_s}
\newcommand{\locdectheta}{\mathbf{\theta}_{\text{dec}_s}}

\newcommand{\contdec}{Dec_c}
\newcommand{\contdectheta}{\mathbf{\theta}_{\text{dec}_c}}

\newcommand{\unit}{\mathbf{a}}
\newcommand{\spfuc}{\phi}
\newcommand{\theofuc}{\mathbf{\Psi}}
\newcommand{\theomat}{\mathbf{C}}

\newcommand{\pemlp}{\mathbf{NN}}

\newcommand{\locdecmlp}{\mathbf{NN}_{\text{dec}}}

\newcommand{\loc}{loc}
\newcommand{\cont}{cont}

\newcommand{\aodha}{wrap}
\newcommand{\naive}{direct}

\newcommand{\numresnet}{h}
\newcommand{\numneuron}{o}

\newcommand{\nilao}[1]{\textcolor{red}{{#1}}}


\newcommand{\mai}[1]{\textcolor{red}{{#1}}}



==> Location Encoding Paper - ICLR 2020/encoder.tex <==
\vsubsection{Encoder}  
\label{sec:encoder}

\paragraph{Point Feature Encoder}          \label{sec:feenc}
%It is a common case that 
Each point $p_i=(\bx_i, \bv_i)$ in a point set $\mP$ is often associated with  features  such as the air pollution station data associate with some air quality measures, a set of POIs with POI types and names, a set of points from survey and mapping with elevation values, a set of points from geological survey with mineral content measure, and so on.  
%represented as $\bv_i$. 
The point feature encoder $\enc^{(v)}()$ encodes such features $\bv_i$ 
%associated with each point 
into a feature embedding $\feemb{i} \in \Real^{\fedim}$. The implementation of $\enc^{(v)}()$ depends on the nature of these features. For example, if each point represents a POI with multiple POI types (as in this study), the feature embedding $\feemb{i}$ can simply be the mean of each POI types' embeddings 
%(See Equ. \ref{equ:feemb}). 
%\begin{equation}
$
\feemb{i} = \dfrac{1}{H} \sum_{h=1}^{H} \mathbf{t}_{h}^{(\gamma)},
$
%\label{equ:feemb}
%\end{equation}
%In Equ. \ref{equ:feemb}, 
where $\mathbf{t}_{h}^{(\gamma)}$ indicates the $h$th POI type embedding of a POI $p_i$ with $H$ POI types.
%More complex encoder for more diverse feature types can be explore in the future.
%To help with  training %}
We apply $L_{2}$ normalization %can be applied 
to the POI type embedding matrix.

\paragraph{Point Space Encoder}  \label{sec:peenc}
A part of the novelty of this paper is from the point space encoder $\enc^{(x)}()$. 
%A contribution 
%A goal
%of this work is to build theoretical models. %such as %\citet{gao2018learning} into general purpose deep models for real world problems. 
We first introduce Theorem \ref{the:gc} which provide an analytical solution $\spfuc(\bx)$ as the base of encoding any location $\bx \in \Real^2$ in 2D space to a distributed representation: %~\citep{gao2018learning}.
\begin{theorem}
	\label{the:gc}
	Let $\theofuc(\bx) = (e^{i\langle \unit_j, \bx \rangle}, j=1,2,3)^T \in \Complex^3$ where $e^{i\theta} = \cos\theta + i\sin\theta$ is the Euler notation of complex values; $\langle \unit_j, \bx \rangle$ is the inner product of $\unit_j$ and $\bx$. $\unit_1, \unit_2, \unit_3 \in \Real^2$ are 2D vectors such that the angle between $\unit_k$ and $\unit_l$ is $2\pi/3$, $\forall j, \|\unit_j\| = 2\sqrt{\alpha}$. Let $\theomat \in \Complex^{3 \times 3}$ be a random complex matrix such as $\theomat^{*}\theomat = \mathbf{I}$. Then $\spfuc(\bx) = \theomat\theofuc(\bx)$, $M(\Delta\bx) = \theomat diag(\theofuc(\Delta\bx))\theomat^{*}$ satisfies 
	\begin{equation}
	%\begin{split}
		\spfuc(\bx+\Delta\bx) = M(\Delta\bx)\spfuc(\bx)
		\label{equ:theo1}\\
	\end{equation} and
	\begin{equation}
	\langle \spfuc(\bx+\Delta\bx), \spfuc(\bx) \rangle = d(1-\alpha\|\Delta\bx\|^2)
	\label{equ:theo2}
	%\end{split}
	\end{equation}
	where $d=3$ is the dimension of $\spfuc(\bx)$ and $\Delta\bx$ is a small displacement from $\bx$.
\end{theorem}
The proof of Theorem \ref{the:gc} can be seen in
\citet{gao2018learning}. $\spfuc(\bx) = \theomat\theofuc(\bx) \in \Complex^3$ amounts to a 6-dimension real value vector and each dimension shows a \textit{hexagon} firing pattern which models the grid cell behavior. 
%According to \citet{gao2018learning}, 
Because of the periodicity of $sin()$ and $cos()$, this single scale representation  $\spfuc(\bx)$ does not form a global codebook of 2D positions, i.e. there can be $\bx \neq \by$, but $\spfuc(\bx) = \spfuc(\by)$. 
%That means $\spfuc(\bx)$ does not encode $\bx$ uniquely. 
%So we combine multiple $\spfuc(\bx)$ with different periodicity to resolve the global ambiguity.

Inspired by Theorem \ref{the:gc} and the multi-scale periodic representation of grid cells in mammals~\citep{abbott2014nobel}
%for coding space, 
we set up our point space encoder $\peemb{} = \enc_{theory}^{(x)}(\bx)$ to use sine and cosine functions of different frequencies to encode positions in space.
%the position component of points. 
%Given a point $p=(\bx, \bv) \in \mP$ or 
Given any point $\bx$ in the studied 2D space, 
% we encode $\bx$ into a $\pedim= 6\nscale$ dimension embedding,  
% where $\nscale$ is the number of grid scales.
the space encoder $\enc_{theory}^{(x)}(\bx) = \pemlp(PE^{(t)}(\bx))$ %\mai{
where $PE^{(t)}(\bx) = [PE^{(t)}_{0}(\bx);...;PE^{(t)}_{s}(\bx);...;PE^{(t)}_{\nscale-1}(\bx)]$
%}
is a concatenation of multi-scale representations of $\pedim= 6\nscale$ dimensions. %\mai{
Here $\nscale$ is the total number of grid scales and $s = 0,1,2,...,{\nscale-1}$.
%}
$\pemlp()$ 
%is a fully connected layer followed by sigmoid activation function. 
% \nilao{
represents fully connected ReLU layers.
% }
Let $\unit_1 = [1,0]^T, \unit_2 = [-1/2,\sqrt{3}/2]^T, \unit_3 = [-1/2,-\sqrt{3}/2]^T \in \Real^2$ be three unit vectors and the angle between any of them is $2\pi/3$. 
%$\bx^{[l]}$ and $\unit_{j}^{[l]}$ indicate the $l$-th dimension of $\bx$ and $\unit_{j}$ respectively. 
% \mai{
$\lambda_{min}, \lambda_{max}$ are the minimum and maximum grid scale and $g = \frac{\lambda_{max}}{\lambda_{min}}$.
%}% is the common ratio of the geometric series of different grid scales; 
At each  scale $s$, $PE^{(t)}_{s}(\bx) = [PE^{(t)}_{s,1}(\bx);PE^{(t)}_{s,2}(\bx);PE^{(t)}_{s,3}(\bx)]$ is a concatenation of three components, where
% $PE^{(t)}_{s,j}(\bx)$ 
%which is computed as 
%Equ. \ref{equ:petheory}. Here 
% \begin{align}
% PE^{(t)}_{s,j}(\bx) = [
% \cos(\frac{\bx^{[l]}\unit_{j}^{[l]}}{ \freq^{s/\nscale}}); 
% \sin(\frac{\bx^{[l]}\unit_{j}^{[l]}}{ \freq^{s/\nscale}})] \forall l = 1,2 \; \forall j = 1,2,3
% \label{equ:petheory}
% \end{align}
\begin{align}
PE^{(t)}_{s,j}(\bx) = [
\cos(\frac{\langle \bx, \unit_{j} \rangle}{ \lambda_{min} \cdot g^{s/(\nscale-1)}}); 
\sin(\frac{\langle \bx, \unit_{j} \rangle}{ \lambda_{min} \cdot g^{s/(\nscale-1)}})] \forall j = 1,2,3; 
\label{equ:petheory}
\end{align}

%where $F$ represents the largest frequency of sinusoid functions.
%In $\enc_{theory}^{(x)}(\bx) = \pemlp(PE^{(t)}(\bx))$, 
$\pemlp()$ and $PE^{(t)}(\bx)$ are analogies of $\theomat$ and $\theofuc(\bx)$ in Theorem \ref{the:gc}.
%If $\pemlp()$ consist of a block diagonal matrix, we call it $\enc_{theorydiag}^{(x)}(\bx)$.

Similarly we can define another space encoder $\enc_{grid}^{(x)}(\bx) = \pemlp(PE^{(g)}(\bx))$  inspired by the position encoding model of Transformer \citep{vaswani2017attention}, where $PE^{(g)}(\bx) = [PE^{(g)}_{0}(\bx);...;PE^{(g)}_{s}(\bx);...;PE^{(g)}_{\nscale-1}(\bx)]$ is still a concatenation of its multi-scale representations, while $PE^{(g)}_{s}(\bx)=[PE^{(g)}_{s,1}(\bx);PE^{(g)}_{s,2}(\bx)]$ 
%is a concatenation of space encoding  which 
handles %\mai{
each component $l$ of $\bx$ 
%, denoted as $\bx^{[l]}$}, 
separately:
%}
%\footnote{\mai{Here $\bx^{[l]}$ indicates the $l$-th dimension of $\bx$.}}
% \begin{align}
% PE^{(g)}_{s,l}(\bx) = [
% \cos(\frac{\bx^{[l]}}{ \freq^{s/\nscale}}); 
% \sin(\frac{\bx^{[l]}}{ \freq^{s/\nscale}})] \forall l = 1,2
% \label{equ:pegrid}
% \end{align}
\begin{align}
PE^{(g)}_{s,l}(\bx) = [
\cos(\frac{\bx^{[l]}}{ \lambda_{min} \cdot g^{s/(\nscale-1)} }); 
\sin(\frac{\bx^{[l]}}{ \lambda_{min} \cdot g^{s/(\nscale-1)} })] \forall l = 1,2
\label{equ:pegrid}
\end{align}

%\nilao{this is implementation detail}
% Since $\sin(\theta)$ can be derived by shifting $\cos(\theta)$ $\pi/4$ in one period, we simply reproduce another space encoder $\enc_{hexa}^{(x)}(\bx) = \pemlp(PE^{(h)}(\bx))$ by changing Equ. \ref{equ:pegrid} to Equ. \ref{equ:pehexa}.
% \begin{align}
% PE^{(h)}_{s,l}(\bx) = [
% \cos(\frac{\bx^{[l]}}{ \freq^{s/\nscale}}); 
% \cos(\frac{\bx^{[l]}}{ \freq^{s/\nscale}} + \frac{2\pi}{3});
% \cos(\frac{\bx^{[l]}}{ \freq^{s/\nscale}} + \frac{4\pi}{3})] \forall l = 1,2
% \label{equ:pehexa}
% \end{align}


==> Location Encoding Paper - ICLR 2020/exp.tex <==
\vsection{Experiment}   \label{sec:exp}
In this section we compare \modelname with commonly used position encoding methods, and analyze them both quantitatively and qualitatively. 
%We compare \modelname to poplar coordinate encoding approaches including
%\vsubsubsection
\paragraph{Baselines}
Our baselines include
1) $\model{\naive}{loc}$  directly applying feed-forward nets \citep{chu2019geo};
2) $\model{tile}{loc}$ discretization \citep{berg2014birdsnap,adams2015frankenplace,tang2015improving};
3) $\model{\aodha}{loc}$
feed-forward nets with coordinate wrapping
 \citep{mac2019presence}; and 
4) $\model{rbf}{loc}$ Radial Basis Function (RBF) kernels \citep{baudat2011kernel,Bierens1994regression}.
See Appendix~\ref{sec:baselines} for details of the baselines.

\vsubsection{POI Type Classification Tasks} \label{sec:poi_type_class}
%\vsubsubsection
\paragraph{Dataset and Tasks}\label{sec:dataset}
To test the proposed model, we conduct experiments on geographic datasets with POI position and type information. 
We utilize the open-source dataset published by Yelp Data Challenge and select all POIs within the Las Vegas downtown area\footnote{The geographic range is (35.989438, 36.270897) for latitude and (-115.047977, -115.3290609) for longitude.}. 
There are 21,830 POIs with 1,191 different POI types 
%(such as \textit{Museum}, \textit{Hotel}, \textit{Nightclub}) 
in this dataset. 
Note that each POI may be associated with one or more types, and we do not use any other meta-data such as business names, reviews for this study.
% As described in Section~\ref{sec:encoder} we associate each POI type with an embedding, and use the average  embedding of associate types as the feature representation for each POI.
We  project  geographic coordinates into projection coordinates  using the NAD83/Conus Albers projection coordinate system\footnote{\url{https://epsg.io/5070-1252}}. 
%Fig. \ref{fig:poi} shows the spatial distribution of these POIs with a basemap. 
The POIs are split into training, validation, and test dataset with ratios 80\%:10\%:10\%. 
%All models are implemented in PyTorch. % and trained on a Linux machine with 4 CPU cores.
We create two tasks setups which represent different types of modeling need in %\mai{
Geographic Information Science:%}
%\nilao{might need more detail here}
\begin{itemize}
\item \textbf{Location Modeling} % \mai{($\loc$)}
predicts %\mai{
the feature information associated with a POI
%}
based on its location $\bx_i$ represented by the \textit{location decoder} $\locdec()$. %\mai{
This represents a large number of location prediction problems such as image fine grained recognition with geographic prior \citep{chu2019geo}, and %location based 
species potential distribution prediction \citep{zuo2008geosvm}.
%, and so on.
%}
\item  \textbf{Spatial Context Modeling} %\mai{($\cont$)}
predicts %\mai{
the feature information associated with a POI
%}
based on its context 
$\{\emb_{i1},...,\emb_{ij},...,\emb_{i\neisize}\}$ represented by the \textit{spatial context decoder} $\contdec()$. %\mai{
This represents a collections of spatial context prediction problem such as spatial context based facade image classification \citep{yan2018xnet+}, and all spatial interpolation problems.
%}
\end{itemize}

% \item Given a point $p_i=(\bx_i, \bv_i)$ a \textbf{point space encoder} $\enc^{(x)}()$ encodes location $\bx_i$ into a location embedding $\peemb{i} \in \Real^{\pedim}$ and a \textbf{point feature encoder} $\enc^{(v)}()$ encodes its feature into a feature embedding $\feemb{i} \in \Real^{\fedim}$.  
% $\emb = [\peemb{i};\feemb{i}] \in \Real^{\embdim}$ is the full representation of point $p_i \in \mP$, where $\embdim = \pedim+\fedim$. 
% $[;]$ represents vector concatenation. 
% While for a point $p_j \notin \mP$ in the studied space, it only has location embedding $\peemb{j}$ since it does not have feature $\bv_i$, or its feature is unknown.
% \item 
% A \textbf{location decoder} $\locdec()$  reconstructs point feature embedding $\feemb{i}$ given location embedding $\peemb{i}$, and 
% a \textbf{spatial context decoder} $\contdec()$ reconstructs the feature embedding $\feemb{i}$ of point $p_i$ based on the space  and feature embeddings $\{\emb_{i1},...,\emb_{ij},...,\emb_{i\neisize}\}$ of 
% neighboring points $\{p_{i1},...,p_{ij},...,p_{i\neisize}\}$, where $\neisize$  is a hyper-parameter. % for the number of neighbours

We use POI  prediction metrics to evaluate these models. Given the real point feature embedding $\feemb{i}$ and $\negsize$ negative feature embeddings $\negsampi = \{\feemb{i}^-\}$, we compare the predicted $\feemb{i}^{\prime}$ with them by cosine distance. The cosine scores are used to rank $\feemb{i}$ and $\negsize$ negative samples. The negative feature embeddings are the feature embeddings of points $p_j$ randomly sampled from $\mP$ and $p_i \neq p_j$. 
We evaluate each model using Negative Log-Likelihood (NLL), Mean Reciprocal Rank (MRR) and HIT@5 (the chance of the true POI being ranked to top 5.
We train and test each model 10 times to estimate standard deviations. 
See Appendix~\ref{sec:parameters} for hyper-parameter selection details.



\vsubsubsection{Location Modeling Evaluation} \label{sec:loceval}
\input{location_result.tex}

We first study location modeling
with the \textbf{location decoder} $\locdec()$ in Section \ref{sec:contdec}.
%test the location model $\modelname^{loc}$ which uses the location decoder model in Sec. \ref{sec:locdec}. 
%
We use a negative sample size of  $\negsize = 100$.
%for training, vaidation, and testing. 
%We also compare different coordinate system with two axis of $90$ degree apart $\model{grid}{loc}$ or three axis of $120$ degree apart  $\model{hexa}{loc}$.
%
Table \ref{tab:loceval} shows the average metrics of different models %\mai{
with their best hyper-parameter setting
%}
on the validation set. 
%
% The figures in () besides MRR/HIT@5 scores indicate the standard deviations of each metric \mai{while () besides the model names indicates the best hyper-parameter of the corresponding models}. \mai{We also list the performances of $\model{theory}{loc}$ with three different $\lambda_{min} = (1k,500,50)$.}
%$NLL$ represents the negative log likelihood. 
%Table \ref{tab:loceval} 
%
We can see that 
%all the \modelname  models outperform $\model{random}{loc}$ selection and 
 $\model{\naive}{loc}$  and
 $\model{theorydiag}{loc}$ are less competitive, only beating the $\model{random}{loc}$ selection baseline.
%on both validation and test dataset.
%
%$\model{theory}{loc}$ almost triple MRR and quadruple HIT@5 on the test dataset with a fare margin.
%statistical significance.
%\nilao{the naive may be too naive?}
Other methods with single scale representations -- including
 $\model{tile}{loc}$, $\model{\aodha}{loc}$, and $\model{rbf}{loc}$ -- perform better.
The best results come from various version of the grid cell models, which are capable of dealing with multi-scale representations.
% and  shows lower performance. $\model{theory}{loc}$ with $\lambda_{min}=50$ has the best performance with 20\%, 21\%, 17\% relative improvement on MRR compared with the best $\model{tile}{loc}$, $\model{\aodha}{loc}$, $\model{rbf}{loc}$. 
%It is a bit surprise that simple $\model{tile}{loc}$  approach outperforms  $\model{\aodha}{loc}$ while \citet{mac2019presence} shows otherwise.
 
 %The performance of $\model{\naive}{loc}$ is similar to that of $\model{random}{}$, a random guessing lower bound. %This shows that we can not directly use raw coordinates to do prediction in this task. 




%\mai{
In order to understand the reason for the superiority of
grid cell models
%$\model{theory}{loc}$  %over $\model{rbf}{loc}$ and other baseline models, we provide empirical analysis. 
 we provide qualitative analysis of their representations.
We apply hierarchical clustering to the  location embeddings produced by studied models
% $\enc_{\naive}^{(x)}(\bx)$, $\enc_{tile}^{(x)}(\bx)$ ($c=500$),
% $\enc_{wrap}^{(x)}(\bx)$ ($\numresnet=3,\numneuron=512$),
% $\enc_{rbf}^{(x)}(\bx)$ ($\sigma=1k$), and $\enc_{theory}^{(x)}(\bx)$ with 3 different $\lambda_{min}$ 
using cosine distance as the distance metric (See Fig. \ref{fig:loc_cluster}).
% \footnote{The spatial resolution is 250 meter $\times$  250 meter.}. 
%
% We also visualize the response maps of the first 8 neurons in the last layer of the corresponding %$\enc_{rbf}^{(x)}(\bx)$ and three $\enc_{theory}^{(x)}(\bx)$ 
% models in  Fig. \ref{fig:locneuron}.} %(See Appendix for all the maps). 
% \mai{By comparing the clustering results and response maps of different models in Fig. \ref{fig:loc_cluster}, \ref{fig:locneuron} and referring to their performance in Table \ref{tab:loceval}, 
we can see that when restricted to large grid sizes ($\lambda_{min} = 1k$), $\model{theory}{loc}$ has similar representation (Fig.~\ref{fig:rbfcluster}, \ref{fig:theory1k}, and Fig.~\ref{fig:locrbf}, \ref{fig:loctheory1k}) and performance compared to $\model{rbf}{loc}$ ($\sigma=1k$). However it is able to significantly outperform $\model{rbf}{loc}$ ($\sigma=1k$) (and $\model{tile}{loc}$ and $\model{\aodha}{loc}$) when small grid sizes ($\lambda_{min} = 500, 50$) are available. The relative improvements over $\model{rbf}{loc}$ ($\sigma=1k$) are -0.2\%, +0.6\%, +2.1\% MRR for $\lambda_{min}$=1k, 500, 50 respectively. 
%}

%We compare the performance of two $\model{theory}{loc}$ models with $\lambda_{min}=$ 50 and 500 on different types of POIs. We found that the biggest improvements come from POI types with concentrated distributions such as women's clothing, restaurants, nightclubs, bars while there is no or negative improvements on POI types with even distributions (e.g., education, hospital, schools, pet and financial services). This result is well aligned with the previous  result about different spatial distribution patterns of different POI types \citep{mckenzie2015poi}. 
%This result indicates that \textbf{the overall performance improvement of $\model{theory}{loc}$ ($\lambda_{min}=50$) is caused by the usage of smaller grid cell sizes in space encoding which can discriminates POI types which tend to cluster together}. 
%Different types of POIs have spatial characteristics at different scales.
%Smaller grid cells can discriminate POI types which tend to cluster together. In contrast, when $\model{rbf}{loc}$  uses a smaller $\sigma$ (and more anchors) or  $\model{tile}{loc}$ uses smaller tile sizes their number of  parameters grows quickly, thus leading to overfitting.

% , the gaussian kernels centered at those RBF anchor points will cover less area while POIs in most of the study area will get near 0 values in all dimensions for the initial RBF space encoding which results in a lower performance. 
% That means \textbf{$\model{theory}{loc}$ beats $\model{rbf}{loc}$ by modeling structures at different scales}. One may be able to design a hierarchically structured RBF which integrates representation of different scales, but that is beyond the scope for this paper.}

%In terms of $\model{\naive}{loc}$ and $\model{\aodha}{loc}$ ($\numresnet$=3,$\numneuron$=512) (See Fig. \ref{fig:naivecluster} and \ref{fig:aodhacluster}), although they can capture the spatial feature distribution, the captured pattern is more coarse and its performances are less than all other models in Fig. \ref{fig:loc_cluster}. This is highly likely because it does not utilize the multi-scale periodic representation and cannot capture the spatial feature distribution at different scales. As for $\model{tile}{loc}$, Fig. \ref{fig:tilecluster} shows clustering result of the best $\model{tile}{loc}$ model ($c=500$) which shows less spatial continuity but still have some similarity with Fig.~\ref{fig:rbfcluster}, \ref{fig:theory1k}. When using smaller $c$ (50), fewer POIs will fall into one grid which makes the model easier to overfit.

%We can see that $\model{rbf}{loc}$ and $\model{theory}{loc}$ ($\lambda_{min}=1k$) have similar firing patterns where different neurons fire at different parts of the city. As $\lambda_{min}$ becomes smaller ($\lambda_{min}=500,50$), the performance of $\model{theory}{loc}$ improves significantly and we start to see grid cell-like firing patterns in their response maps while the neurons stills fires at different locations but in a more fractured way. This indicates $\model{theory}{loc}$ with smaller $\lambda_{min}$ is able to capture the feature distribution in a finer scale.

%In order to understand the reason why our location models perform well, we first visualize the response maps of the first 8 neurons in the last layer of $\enc_{\naive}^{(x)}(\bx)$ and $\enc_{theory}^{(x)}(\bx)$ in  Fig. \ref{fig:locneuron} (See Appendix for all the maps). 
%From Fig. \ref{fig:locneuron}, we can see that the response map of $\enc_{\naive}^{(x)}(\bx)$ is almost random even we train each model 2000 iterations until the model coverages. However, the response map of $\enc_{theory}^{(x)}(\bx)$ is very interesting. For example, Neuron 0 only fires at the city center of Las Vegas while Neuron 8 shows the opposite patterns. 
%It would be interesting to study the similarity and difference of them
%This response maps are similar
%to the performance of place cells in Neurioscience research. 
%Our explanation is that $\enc_{theory}^{(x)}(\bx)$ first decomposes the locations of points into multi-scale periodical representations and these representations reserve the spatial adjacency information according to Theorem \ref{the:gc}. So $\pemlp()$ is easier to understand the spatial proximity information. In contrast, the raw coordinates do not have a linear relationship and hard for $\pemlp()$ to understand. 


%Next, we use hierarchical clustering to cluster these location embeddings produced by $\enc_{\naive}^{(x)}(\bx)$ and $\enc_{theory}^{(x)}(\bx)$ with cosine distance as the distance matric which are shown in Fig. \ref{fig:naivecluster} and \ref{fig:theorycluster}\footnote{The spatial resolution is 250 meter $\times$  250 meter.}. We can see that the clustering result of $\enc_{\naive}^{(x)}(\bx)$ is almost random but that of $\enc_{theory}^{(x)}(\bx)$ shows a block-like clustering pattern. When we compare it with Fig. \ref{fig:poi}, we find out these clustering patterns reflect the urban structures. %This is also related to the concept of semantic signature \citep{janowicz2019using} in GIS research.


\input{locmodel_stats.tex}

\vsubsubsection{Spatial Context Modeling Evaluation}  \label{sec:conteval}
\input{context_result.tex}

Next, we evaluate the 
%performance of the spatial context model $\modelname^{cont}$ which uses the spatial context decoder model 
 \textbf{spatial context decoder} $\contdec()$ in Sec. \ref{sec:contdec}. 
%
We use the same evaluation set up as location modeling. 
The context points are obtained by querying the $\neisize$-th nearest points  using PostGIS ($\neisize = 10$). 
As for validation and test datasets, we make sure the center points are all unknown during the training phase. 
%See Appendix~\ref{sec:parameters} for hyper-parameter selection details.
Table \ref{tab:conteval} shows the evaluation results of different models
%on the validation and test datasets 
for spatial context modeling. 
%Similar to Sec. \ref{sec:conteval}, we also run each model 10 times and report the average score for each metric. 
%We can see that all of our multi-scale periodic representation based model outperform $\model{none}{cont}$, $\model{\naive}{cont}$, $\model{polar}{cont}$, and $\model{rbf}{cont}$ with a fare margin except $\model{theorydiag}{cont}$ while $\model{hexa}{cont}$ shows the best performance with 4\% relative improvement of MRR on the test dataset over $\model{rbf}{cont}$. 
The baseline approaches %to location modeling
($\model{\naive}{cont}$, $\model{tile}{cont}$,  $\model{\aodha}{cont}$, $\model{rbf}{cont}$) generally perform poorly in context modeling.
% task which models relative positions of POIs.
We designed specialized version of these approaches ($\model{polar}{cont}$,  $\model{polar\_tile}{cont}$, $\model{scaled\_rbf}{cont}$) with polar coordinates, which lead to significantly improvements.
Note that these are  models proposed by us specialized for context modeling and therefore are less general than the grid cell approaches.
Nevertheless the grid cell approaches
% ($\model{theory}{cont}$ with $\lambda_{min}=10$) 
are able to perform better than the specialized approaches  on the test dataset while have competitive performance on validation dataset.
See Appendix~\ref{sec:apdx:context} for the visualization of context models.
%
% The performances of multiple $\model{theory}{cont}$ with different $\lambda_{min}$ are compared with various specialized baseline models. 
% % (200,100,50,10) are listed in Table \ref{tab:conteval}.
% We can see that $\model{theory}{cont}$ ($\lambda_{min}=10$) can significantly outperform $\model{none}{cont}$, $\model{\naive}{cont}$, $\model{polar}{cont}$, $\model{tile}{cont}$, $\model{polar\_tile}{cont}$, $\model{\aodha}{cont}$, and $\model{rbf}{cont}$. 
% We find $\model{scaled\_rbf}{cont}$ has a similar performance as $\model{theory}{cont}$. 
% Note that $\model{scaled\_rbf}{cont}$ is also a new model proposed by us in order to understand the reason for grid cell models' superiority. 
Actually the gains are small for all baseline approaches also. The reason is that we expect location encoding to be less important when context information is accessible. Similarly as discussed in \citep{gao2018learning}, it is when there is a lack of visual clues that the grid cells of animals are  the most helpful for their navigation. 

\input{context_viz.tex}


\input{img_class.tex}

==> Location Encoding Paper - ICLR 2020/img_class.tex <==
\subsection{Fine-Grained Image Classification Tasks}
To demonstrate the generalizability of  \modelname
%the proposed general purpose representation model 
for space representation
we utilized the proposed point space encoder $\enc^{(x)}()$ model in a well-known computer vision task: \textit{fine-grained image classification}.
%
As we discussed in Section \ref{sec:related}, many studies \citep{berg2014birdsnap,chu2019geo,mac2019presence} have shown that geographic prior information - where (and when) the image is taken - is very important additional information for the fine-grained image classification task and can substantially improve the model performance. 
For example, the appearance information is usually not sufficient to differentiate two visually similar species. 
In this case, the geographic prior becomes much more important because these two species may have very different spatial prior distributions such as the example of European Toads and Spiny Toads in Figure 1 of \citet{mac2019presence}.

We adopt the task setup of \citet{mac2019presence}. During training we have a set of tuples $D = \{(I_{i}, \bx_{i}, y_{i}, p_{i}) \mid i = 1,...,N\}$ where $I_{i}$ indicates an image, $y_{i} \in \{1,2,...,C\}$ is the corresponding class label (species category), $\bx_{i} = [longitude_{i}, latitude_{i}]$ is the geographic coordinates where the image was taken, and $p_{i}$ is the id of the photographer who took this image. At training time, a location encoder is trained to capture the spatial prior information $P(y \mid \bx)$. At inference time, $p_{i}$ information is not available and the final image classification prediction is calculated based on the combination of two models: 1) the trained location encoder which captures the spatial priors $P(y \mid \bx)$ and 2) the pretrained image classification model, InceptionV3 network \citep{szegedy2016rethinking}, which captures $P(y \mid I)$. Bayesian theory has been used to derive the joint distribution $P(y \mid I, \bx)$. See \citet{mac2019presence} for detail explanation as well as the loss function.
%\nilao{
Note that 
%for this task we apply \modelname for density estimation module instead of distributed representation. 
while \modelname outperforms specialized density estimation methods such as Adaptive Kernel \citep{berg2014birdsnap}, it would be interesting  to explore   early fusion \modelname's representations with the image module.
%in the future work.
%}

We use two versions of our point space encoder $\enc^{(x)}()$ model ($grid$, $theory$) as the location encoder to capture the spatial prior information $P(y \mid \bx)$. The evaluation results of our models as well as multiple baselines are shown in Table \ref{tab:imgcls_eval}. We can see that \textbf{both $grid$, $theory$ outperform previous models as well as that of \citet{mac2019presence}   on two fine-grained image classification datasets  with significant sizes: BirdSnap$\dagger$, NABirds$\dagger$}. $theory$ shows superiority over $grid$ on NABirds$\dagger$ while fail to outperform $grid$ on BirdSnap$\dagger$. Note that we only pick baseline models which capture spatial-only prior and drop models which additionally consider time information. Both $grid$ and $theory$ use 1 hidden ReLU layers of 512 neurons for $\mathbf{NN}()$ and they have the same hyperparameters: $\lambda_{min}$=0.0001, $\lambda_{max}$=360, $\nscale$ = 64. Like \citet{mac2019presence}, the location embedding size $\pedim$ is 1024 and we train the location encoder for 30 epochs. Our implementation is based on the original code\footnote{\url{https://github.com/macaodha/geo_prior/}} of \citet{mac2019presence} for both model training and evaluation phase.




%\begin{table}[]
%	\caption{The fine-grained image classification accuracy of different models on three datasets: BirdSnap, BirdSnap$\dagger$, NABirds$\dagger$. The classification accuracy is calculated by combining image classification predictions $P(y \mid I)$ with different spatial priors $P(y \mid \bx)$. The $grid$ and $theory$ model use 1 hidden ReLU layers of 512 neurons. The evaluation results of the baseline models are taken from Table 1 of \citet{mac2019presence}. See more detail about the datasets and task setup from \citet{mac2019presence}.}
%	\label{tab:imgcls_eval}
%	\centering
%	\small{
%		\begin{tabular}{l|l|l|l}
%			\toprule
%			& BirdSnap       & BirdSnap$\dagger$      & NABirds$\dagger$       \\ \hline
%			$P(y \mid \bx)$ - Prior Type         & Test           & Test           & Test           \\ \hline
%			No Prior (i.e. uniform)     & 70.07          & 70.07          & 76.08          \\
%			Nearest Neighbor (num)      & 70.82          & 77.76          & 79.99          \\
%			Nearest Neighbor (spatial)  & 71.57          & 77.98          & 80.79          \\
%			Discretized Grid            & 71.13          & 77.19          & 79.58          \\
%			Adaptive Kernel \citep{berg2014birdsnap}     & 71.57          & 78.65          & 81.11          \\
%			$\aodha$ \citep{mac2019presence}  (no date) & 71.66          & 78.65          & 81.15          \\ \hline
%			$grid$ ($\lambda_{min}$=0.0001, $\lambda_{max}$=360, $\nscale$ = 64)  & 71.62          & \textbf{79.44} & 81.28          \\
%			$theory$ ($\lambda_{min}$=0.0001, $\lambda_{max}$=360, $\nscale$ = 64) & \textbf{71.97} & 79.35          & \textbf{81.59} \\
%			\bottomrule
%		\end{tabular}
%	}	\vspace*{-0.25cm}
%\end{table}

\begin{table}[t!]
	\caption{Fine-grained image classification results on two datasets: BirdSnap$\dagger$ and NABirds$\dagger$. The classification accuracy is calculated by combining image classification predictions $P(y \mid I)$ with different spatial priors $P(y \mid \bx)$. The $grid$ and $theory$ model use 1 hidden ReLU layers of 512 neurons. The evaluation results of the baseline models are  from Table 1 of \citet{mac2019presence}. 
	%See more detail about the datasets and task setup from \citet{mac2019presence}.
	}
	\label{tab:imgcls_eval}
	\centering
	\small{
		\begin{tabular}{l|l|l}
			\toprule
			& BirdSnap$\dagger$      & NABirds$\dagger$       \\ \hline
			%		$P(y \mid \bx)$ - Prior Type         & Test           & Test           \\ \hline
			No Prior (i.e. uniform)     & 70.07          & 76.08          \\ \hline
			Nearest Neighbor (num)      & 77.76          & 79.99          \\
			Nearest Neighbor (spatial)  & 77.98          & 80.79          \\ \hline
			Adaptive Kernel \citep{berg2014birdsnap}     & 78.65          & 81.11          \\
			%Discretized Grid 
			$tile$
			\citep{tang2015improving} (location only)         & 77.19          & 79.58          \\
			$\aodha$ \citep{mac2019presence}  (location only) & 78.65          & 81.15          \\ %\hline
			$rbf$ ($\sigma$=1k)     & 78.56 & 81.13          \\
			$grid$ ($\lambda_{min}$=0.0001, $\lambda_{max}$=360, $\nscale$ = 64)  & \textbf{79.44} & 81.28          \\
			$theory$ ($\lambda_{min}$=0.0001, $\lambda_{max}$=360, $\nscale$ = 64) & 79.35          & \textbf{81.59} \\
			\bottomrule
		\end{tabular}
	}	\vspace*{-0.25cm}
\end{table}



==> Location Encoding Paper - ICLR 2020/intro.tex <==
\vsection{Introduction}     \label{sec:intro}

Unsupervised text encoding models such as Word2Vec~\citep{mikolov2013distributed}, Glove~\citep{pennington2014glove}, ELMo~\citep{peters2018deep}, and BERT~\citep{devlin2018bert} have been effectively utilized in many Natural Language Processing (NLP) tasks. 
%The key assumption behind these models is the \textit{distributional semantics } assumption by which  \textit{you shall know a word by the company it keeps} -- 
At their core they
train models which encode words into vector space representations based on their positions in the text and their context. 
A similar situation can be encountered in the field of Geographic Information Science (GIScience). For example, spatial interpolation aims at predicting an attribute value, e.g., elevation,  at an unsampled location based on the known attribute values of nearby samples. 
%The emerging GeoAI field \nilao{citation} also aims to incorporate geographic information such as geographic coordinates into neural networks to make them \textit{spatially explicit}. 
%The computer vision community also shows increasing interests in incorporating geographic information into neural network architectures for multiple tasks such as image classification \citep{tang2015improving} and fine grained recognition \citep{berg2014birdsnap,chu2019geo,mac2019presence}.
Geographic information has become an important component to many  tasks such as fine-grained image classification~\citep{mac2019presence}, 
point cloud classification and semantic segmentation~\citep{qi2017pointnet}, 
reasoning about Point of Interest (POI) type similarity ~\citep{yan2017itdl}, 
land cover classification \citep{kussul2017deep},
% weather forecasting,  
%air pollution prediction~\citep{lin2018exploiting}, 
%traffic forecasting~\citep{li2017diffusion}, 
%traffic congestion prediction \citep{polson2017deep}, 
% autonomous driving controlling, 
%geographic knowledge graph summarization \citep{yan2019spatial}, 
and geographic question answering \citep{mai2019relaxing}.
% \nilao{
Developing a \textit{general} model for 
%spatial density estimation 
vector space representation of any point in space
would pave the way for many future applications.
%that include a (geo)spatial component.
% }


\begin{figure*}[h!]
	\centering
	\begin{subfigure}[b]{0.19\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./fig/womens_cloth.png}
		\subcaption[]{Women's Cloth}
		%{{\small  $\enc_{\naive}^{(x)}(\bx)$}}    
		\label{fig:women_cloth}
	\end{subfigure}
	\begin{subfigure}[b]{0.19\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./fig/education.png}
		\subcaption[]{Education
		}
		%{{\small  $\enc_{\naive}^{(x)}(\bx)$}}    
		\label{fig:education}
	\end{subfigure}
	%\hfill
% 	\vspace*{-0.05cm}
	\begin{subfigure}[b]{0.282\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/ripleys_k.png}
		\subcaption[]{Ripley's K
		}
		\label{fig:ripley}
	\end{subfigure}
	\vspace*{-0.05cm}
	\begin{subfigure}[b]{0.31\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./fig/ripleys_k_log.png} %\vspace{-0.01cm}
		\subcaption[]{Renormalized Ripley's K% (log)
		}
		\label{fig:ripley_log}
	\end{subfigure}
	%\hfill

	\vspace*{-0.05cm}
	\caption{\small
	The challenge of joint modeling distributions with very different characteristics.
	(a)(b)  The POI locations (red dots) in Las Vegas and \modelname predicted conditional likelihood of 
	Women's Clothing (with a clustered distribution) and 
    Education (with an even distribution). The dark area in (b) indicates that the downtown area has more POIs of  other types   than  education.
    %is dumped when conditioned over all types.
    %\footnote{Note that because the response map shows the \textit{conditional} likelihood, Fig. \ref{fig:education} shows rather dark in Las Vegas downtown area.}; 
	(c)  Ripley's K curves of POI types for which \modelname has the largest and smallest improvement over  $\aodha$ \citep{mac2019presence}. Each curve  represents  the number of POIs of a certain type inside certain radios centered at every POI of that type; 
	(d)  Ripley's K curves renormalized by POI densities and shown in log-scale. 
%	Multi-scale representation 	is necessary to jointly describe the spatial density estimation surface of these two types of POI distributions.%: concentrated and even distributions.
	To efficiently achieve multi-scale representation \modelname concatenates the grid cell encoding of 64 scales (with wave lengths ranging from 50 meters to $40k$ meters) as the first layer of a deep model, and trains with POI data in an unsupervised fashion.
	}
	\label{fig:motivation}
	\vspace*{-0.5cm}
\end{figure*}


However, existing models often utilize \textit{specific} methods to deal with geographic information  and often disregards geographic coordinates. 
For example, Place2Vec~\citep{yan2017itdl} converts the coordinates of POIs into spatially collocated POI pairs within certain distance bins, and does not preserve information about the (cardinal) direction between points. % in model training. 
\citet{li2017diffusion} propose 
%Diffusion Convolutional Recurrent Neural Network (DCRNN) 
DCRNN for traffic forecasting in which the traffic sensor network is converted to a distance weighted graph which necessarily forfeits information about the spatial layout of sensors.
There is, however, no general representation  model 
%that could be used as a common building block. 
 beyond simply applying discretization  \citep{berg2014birdsnap, tang2015improving}  or feed-forward nets \citep{chu2019geo,mac2019presence} to coordinates.
 

%Hence, in this paper, we propose \textit{a space encoding model, that learns the probability distribution of point features over space and facilitates distributed representation learning of any point. % in the modeled space.} 
%Such a model will be valuable for POI search, vector-based spatial interpolation, geo-tagged image classification, spatial embedded social network classification, air pollution or traffic forecasting, and so on. 
%As far as we know, there is no such general purpose space encoding model exists and this is the major objective of this paper.


% \nilao{
A key challenge in developing a general-purpose representation model for space is how to deal with mixtures of distributions with very different characteristics (see an example in  Figure~\ref{fig:motivation}), which often emerges in spatial datasets~\citep{mckenzie2015poi}.
For example, there are POI types with clustered distributions such as women's clothing, %fashion, and Chinese food, 
while there are other POI types with regular distributions such as education. %, pets, pet services.
These feature distributions co-exist in the same space,  and yet we want a single  representation to accommodate all of them in a task such as location-aware image classification~\citep{mac2019presence}.
%
%Fig. \ref{fig:women_cloth}, \ref{fig:education} shows examples of these two distinct spatial distribution patterns: women's cloth (concentrated) and education (even) which are indicated as red dots while the background are the predicted probability distributions of the corresponding POI types by our model.
Ripley's K is a spatial analysis method used to describe point patterns over a given area of interest.
Figure \ref{fig:ripley} shows the K plot of several POI types in Las Vegas. One can see that as the radius grows the numbers of POIs increase at different rates for different  POI types.
%they have different density at different scales. %
%The black dot line indicates the theoretical Poisson distribution. It shows that the Ripley's K lines of pet, pet services, and education are very flat and similar to each other while the lines of women's cloth, fashion, Chinese food are rather far way from them. 
%This indicates the last three POI types have more concentrated distributions. 
%Note that the Ripley's K lines are focusing on the point density at different scales (buffer radios).
In order to see the relative change of density at different scales, 
we renormalize the curves by each POI type's density and show it in log scale in Figure~\ref{fig:ripley_log}.
%is the renormalized Ripley's K plot in log-scale where 
%we can see that the lines of women's cloth, fashion, and Chinese food begin with a very flat slope and become steep later while the other three POI types have a rather steep line in the beginning. 
One can see two distinct POI type groups with different distribution patterns with
%\footnote{Since we renormalize the Ripley's K lines by the POI densities, the poisson distribution will have a steep line with constant slope.}: 
clustered and even distributions. 
If we want to model the distribution
%density estimation surface 
of these POIs by discretizing the study area into tiles, 
%in order to precisely describe the concentrated distributed POI types such as women's clothing, 
we have to use small grid sizes for women's clothing
%while as for those even distributed POI types such as education, we may want to 
while using larger grid sizes for educations because smaller grid sizes lead to over-	parameterization of the model and overfitting. 
In order to 
%build a general purpose space representation model which can 
jointly describe these distributions and their patterns, we need an encoding method which supports \textit{multi-scale representations}.
% }

Nobel Prize winning Neuroscience research~\citep{abbott2014nobel} has demonstrated that grid cells in mammals provide a multi-scale periodic representation that functions as a metric for location encoding, which is critical for integrating self-motion. 
%The discovery of grid cells %\citep{mcnaughton2006path,burak2009accurate} and place cells~\citep{samsonovich1997path} assists researchers to understand how the brains of mammals represent the \textit{absolute} and \textit{relative} positions in an environment. 
%In fact, for cognitive tasks, neural systems often need to maintain certain internal representations of relevant variables in the absence of external stimuli \citep{cueva2018emergence}. 
Moreover, \citet{blair2007scale} show that the multi-scale periodic representation of grid cells can be simulated by summing three cosine grating functions oriented $60^{\circ}$ apart, which may be regarded as a simple Fourier model of the hexagonal lattice. 
% \nilao{ 
This research inspired us to encode locations with multi-scale periodic representations. 
Our assumption is that decomposed geographic coordinates 
%are  easier to learn within 
helps 
machine learning models, such as deep neural nets,
and  multi-scale representations deal with the inefficiency of intrinsically single-scale methods such as RFB kernels or discretization (tile embeddings). 
% }
To validate this intuition, we propose an encoder-decoder framework to encode the distribution of point-features\footnote{In GIS and spatial analysis, `features' are representations of real-world entities. A tree can, for instance, be modeled by a point-feature, while a street would be represented as a line string feature.} in space and train such a model in an unsupervised manner. This idea of using sinusoid functions with different frequencies to encode positions is similar to the position encoding proposed in the Transformer model~\citep{vaswani2017attention}. However, the position encoding model of Transformer deals with a discrete 1D space -- the positions of words in a sentence -- while our model works on higher dimensional continuous spaces such as the surface of earth. 

\textbf{In summary, the contributions of our work are as follows:}% as follows:}
\begin{enumerate}
	\item We propose an encoder-decoder encoding framework called \modelname using sinusoid functions with different frequencies to model 
	%the distribution of associated features at a location using 
	absolute positions and spatial contexts. %Such an inductive learning model is trained in an unsupervised learning approach.
	%\item 
	We also propose a multi-head attention mechanism
	%based decoder which predicts the center point feature embedding 
	based on context points. 
	To the best of our knowledge, this is the first attention model that explicitly considers the spatial relationships between the query point and context points.
	
	\item 
	We conduct experiments on two real world geographic data for two different tasks:
	1) predicting types of  POIs given their positions and context,
	2) image classification leveraging their geo-locations.
% We conduct two types of experiments on POI type prediction based on 1) the location of the query point
% 	(location modeling)
% 	and 2) its nearby POIs 	(spatial context modeling)
% 	 with real world datasets. 
% 	 Results show that 
	\modelname 
	%our encoding model %significantly 
	outperforms  well-established  encoding methods such as RBF kernels, multi-layer feed-forward nets, and tile embedding approaches for location modeling and image classification.
	%in both tasks. 
	%To the best of our knowledge, this is the first research to use the
	%This is the first time grid cell-like representations achieve superior results in real-world GIS problems compared to well established representations in machine learning.% and deep learning.
	
	\item To understand the advantages of \modelname
	%our proposed approach, 
	we visualize the firing patterns (response maps) of location models' encoding layer neurons and show how they 
	%different neurons of the space encoding layer fire at different locations of the urban environment, which 
	%reflect the underlining urban structure. 
% 	\mai{
	handle spatial structures at different scales by integrating multi-scale representations.
% 	}
	Furthermore the firing patterns for the %\mai{
	spatial context
	%}
	models neurons give insight into how the grid-like cells  
	%represent the relative position of nearby POIs.
% 	\mai{
	capture the decreasing distance effect with multi-scale representations. %\nilao{decreasing distance effect?}
% 	}
\end{enumerate}


==> Location Encoding Paper - ICLR 2020/location_result.tex <==

\begin{figure*}[h!]
	\centering \tiny
	\vspace*{-0.3cm}
	\begin{subfigure}[b]{0.14\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/global_naive_1h512e64.png}\vspace*{-0.1cm}
		\caption[]%
		{{\small 
		%$%\model{rbf}{loc} 
		$\model{\naive}{loc}$
		}}    
		\label{fig:naivecluster}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.137\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/global_tile_500_1h512e64.png}\vspace*{-0.4cm}
		\caption[]%
		{{\small 
		%$%\model{rbf}{loc} 
		$\model{tile}{loc}$ %($c$=500)
		}}    
		\label{fig:tilecluster}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.141\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/global_aodha_3h512e64_none.png}\vspace*{-0.1cm}
		\caption[]%
		{{\small 
		%$%\model{rbf}{loc} 
		$\model{\aodha}{loc}$ %($\numresnet$=3)
		}}    
		\label{fig:aodhacluster}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.145\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/global_rbf_relu_cluster.png}\vspace*{-0.15cm}
		\caption[]%
		{{\small 
		%$%\model{rbf}{loc} 
		$\model{rbf}{loc}$ ($\sigma$=1k)
		}}    
		\label{fig:rbfcluster}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.136\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/global-theory-32-40k-1k-cluster.png}\vspace*{-0.35cm}
		\caption[]%
		{{\small  
		%$\model{theory}{loc} 
		$\lambda_{min}$=1k %, \lambda_{max}=40k$ 
		}}    
		\label{fig:theory1k}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.136\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/global-theory-32-40k-500-cluster.png}\vspace*{-0.35cm}
		\caption[]%
		{{\small  
		%$\model{theory}{loc} 
		$\lambda_{min}$=500 %, \lambda_{max}=40k$ 
		}}    
		\label{fig:theory500}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.142\textwidth}  
		\centering 
		\includegraphics[width=\textwidth]{./fig/global_theory_3h_cluster.png}\vspace*{-0.1cm}
		\caption[]%
		{{\small 
		%$\model{theory}{loc}$ 
		$\lambda_{min}$=50%, \lambda_{max}=40k$ 
		}}    
		\label{fig:theory40}
	\end{subfigure}
	\vspace*{-0.15cm}
	\caption{%Compare 
	\small
	Embedding clustering  of (a) $\model{\naive}{loc}$; (b) $\model{tile}{loc}$ with the best cell size $c=500$; (c) $\model{\aodha}{loc}$ ($\numresnet=3,\numneuron=512$); (d) $\model{rbf}{loc}$ with the best $\sigma$ (1k) and 200 anchor points (red) and (e)(f)(h) $\model{theory}{loc}$ models with different $\lambda_{min}$, but fixed $\lambda_{max}=40k$ and $\nscale = 64$. 
	All models use 1 hidden ReLU layers of 512 neurons except $\model{\aodha}{cont}$. %FFN.
	%The spatial resolution is 250 meter $\times$  250 meter.
% 	$\model{rbf}{loc}$ has issue representing at multi-scale. 
% and in low density areas.
	} 
	\label{fig:loc_cluster}
	\vspace*{-0.15cm}
\end{figure*}
% \begin{figure*}[h!]
% 	\centering \tiny
% 	\begin{subfigure}[b]{0.20\textwidth}
% 		%\centering
% 		\includegraphics[width=\textwidth]{./fig/map.jpg}
% 		\caption[]%
% 		{{\small Las Vegas %downtown
% 		}}    
% 		\label{fig:poi}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[b]{0.26\textwidth}  
% 		\centering 
% 		\includegraphics[width=\textwidth]{./fig/global_naive_g_spa_enc_cluster_new.png}\vspace*{-0.2cm}
% 		\caption[]%
% 		{{\small %Hierarchical Clustering of  
% 		$\model{\naive}{loc}$ %place embeddings.
% 		}}    
% 		\label{fig:naivecluster}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[b]{0.26\textwidth}  
% 		\centering 
% 		\includegraphics[width=\textwidth]{./fig/global_rbf_relu_cluster.png}\vspace*{-0.2cm}
% 		\caption[]%
% 		{{\small %Hierarchical Clustering of 
% 		$\model{rbf}{loc}$
% 		% place embeddings.
% 		}}    
% 		\label{fig:rbfcluster}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[b]{0.26\textwidth}  
% %./fig/global_theory_g_spa_enc_cluster_50_4000_ffn_relu_1_512.png
% 		\centering 
% 		\includegraphics[width=\textwidth]{./fig/global_theory_3h_cluster.png}\vspace*{-0.2cm}
% 		\caption[]%
% 		{{\small %Hierarchical Clustering of 
% 		$\model{theory}{loc}$ %place embeddings.
% 		}}    
% 		\label{fig:theorycluster}
% 	\end{subfigure}
	
% 	\caption{The comparison between the real POI distribution and the clustering results of the space embeddings from two different location models. 
% 	%\nilao{increase resolution for (b)}
% 	} 
% 	\label{fig:poicl}
% 	\vspace*{-0.45cm}
% \end{figure*}



\begin{table}[]
	\caption{The evaluation results of different location models on the validation and test dataset.}
	\label{tab:loceval}
	\centering
	\small{ \begin{tabular}{c|c|ccc|cc}
		\toprule
		\multicolumn{1}{l|}{\multirow{2}{*}{}} & Train & \multicolumn{3}{c|}{Validation}           & \multicolumn{2}{c}{Testing}              \\ 
		%\cline{2-8} 
		\multicolumn{1}{l|}{}  & NLL    & NLL 
		& MRR        & HIT@5  & MRR      & HIT@5  \\ \hline
		$\model{random}{}$ &  & -
		& 0.052 (0.002) & 4.8 (0.5)        
		& 0.051 (0.002) & 5.0 (0.5)  \\ %\hline
		$\model{\naive}{loc}$ %\citep{chu2019geo} 
		& 1.285 & 1.332 %(0.001) 
		& 0.089 (0.001) & 10.6 (0.2)        
		& 0.090 (0.001) & 11.3 (0.2)  \\ %\hline
% 		$\model{gridlookup}{loc}$ ($c$=1k) & 1.197 & 1.283 %(0.001) 
% 		& 0.117 (0.001) & 15.9 (0.3)        
% 		& 0.122 (0.004) & 15.6 (0.6)  \\ %\hline
% 		$\model{gridlookup}{loc}$ ($c$=500) & 1.155 & 1.279 %(0.001) 
% 		& 0.114 (0.001) & 14.1 (0.2)        
% 		& 0.126 (0.001) & 16.8 (0.3)  \\ %\hline
% 		$\model{gridlookup}{loc}$ ($c$=200) & 1.058 & 1.288 %(0.001) 
% 		& 0.119 (0.001) & 16.1 (0.2)        
% 		& 0.121 (0.001) & 16.2 (0.3)  \\ %\hline
% 		$\model{gridlookup}{loc}$ ($c$=50) & 0.946 & 1.433 %(0.001) 
% 		& 0.101 (0.001) & 13.1 (0.2)        
% 		& 0.103 (0.002) & 14.2 (0.4)  \\ \hline
% 		$\model{gridlookupp\_noffn}{loc}$ ($c$=1k) & 1.178 & 1.273 %(0.001) 
% 		& 0.116 (0.001) & 15.6 (0.2)        
% 		& 0.118 (0.001) & 16.3 (0.4)  \\ %\hline
		$\model{tile}{loc}$  %(\cite{tang2015improving})
		($c$=500) 
		& 1.118 & 1.261 %(0.001) %\cite{berg2014birdsnap,adams2015frankenplace,tang2015improving}
		& 0.123 (0.001) & 16.8 (0.2)        
		& 0.120 (0.001) & 17.1 (0.3)  \\ %\hline
% 		$\model{gridlookupp\_noffn}{loc}$ ($c$=200) & 1.039 & 1.265 %(0.001) 
% 		& 0.121 (0.002) & 16.1 (0.3)        
% 		& 0.126 (0.001) & 17.9 (0.2)  \\ %\hline
% 		$\model{gridlookup\_noffn}{loc}$ ($c$=50) & 0.908 & 1.343 %(0.001) 
% 		& 0.113 (0.001) & 14.9 (0.2)        
% 		& 0.115 (0.002) & 15.3 (0.2)  \\ \hline
		
% 		Mac Aodha et al. \cite{mac2019presence} ($1h64e64_n$) & 1.242 & 1.307 %(0.001) 
% 		& 0.098 (0.000) & 12.7 (0.0)        
% 		& 0.101 (0.000) & 13.1 (0.0)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($2h64e64_n$) & 1.239 & 1.302 %(0.001) 
% 		& 0.099 (0.000) & 11.6 (0.0)        
% 		& 0.102 (0.000) & 13.5 (0.0)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($3h64e64_n$) & 1.240 & 1.300 %(0.001) 
% 		& 0.098 (0.000) & 12.5 (0.0)        
% 		& 0.103 (0.000) & 13.1 (0.0)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($4h64e64_n$) & 1.240 & 1.305 %(0.001) 
% 		& 0.102 (0.000) & 12.9 (0.0)        
% 		& 0.103 (0.000) & 13.2 (0.0)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($1h256e64$) & 1.230 & 1.296 %(0.001) 
% 		& 0.102 (0.000) & 13.7 (0.0)        
% 		& 0.103 (0.000) & 13.3 (0.0)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($1h256e64$) & 1.224 & 1.293 %(0.001) 
% 		& 0.104 (0.000) & 13.7 (0.0)        
% 		& 0.110 (0.000) & 14.7 (0.0)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($1h512e64_relu$) & 1.225 & 1.296 %(0.001) 
% 		& 0.108 (0.000) & 14.4 (0.0)        
% 		& 0.114 (0.000) & 14.9 (0.0)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($2h512e64_relu$) & 1.226 & 1.294 %(0.001) 
% 		& 0.107 (0.000) & 13.2 (0.0)        
% 		& 0.112 (0.000) & 15.0 (0.0)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($3h512e64_relu$) & 1.227 & 1.293 %(0.001) 
% 		& 0.108 (0.000) & 13.6 (0.0)        
% 		& 0.111 (0.000) & 13.6 (0.0)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($4h512e64_relu$) & 1.227 & 1.294 %(0.001) 
% 		& 0.105 (0.000) & 14.1 (0.0)        
% 		& 0.110 (0.000) & 14.0 (0.0)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($1h512e64$) & 1.226 & 1.294 %(0.001) 
% 		& 0.109 (0.000) & 13.8 (0.0)        
% 		& 0.113 (0.000) & 15.2 (0.0)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($2h512e64$) & 1.221 & 1.291 %(0.001) 
% 		& 0.108 (0.000) & 14.8 (0.0)        
% 		& 0.115 (0.000) & 15.1 (0.0)  \\ %\hline
		$\model{\aodha}{loc}$% (\cite{mac2019presence}) 
		($\numresnet$=3,$\numneuron$=512) 
		& 1.222 & 1.288 %(0.001) %
		& 0.112 (0.001) & 14.6 (0.1)        
		& 0.119 (0.001) & 15.8 (0.2)  \\ %\hline
% 		Mac Aodha et al. \cite{mac2019presence} ($4h512e64$) & 1.219 & 1.288 %(0.001) 
% 		& 0.111 (0.000) & 14.8 (0.0)        
% 		& 0.114 (0.000) & 14.7 (0.0)  \\ %\hline
    %  	$\model{rbf}{loc}$  & & 1.298 %(0.001) 
    %  	& 0.094 (0.002) & 12.0 (0.4)        
    %  	& 0.090 (0.002) & 11.9 (0.3) \\ %\hline
    %  	$\model{rbf}{loc}$  & 1.268 & 1.296 %(0.001) 
    %  	& 0.095 (0.000) & 12.1 (0.0)        
    %  	& 0.092 (0.000) & 12.3 (0.3) \\ %\hline
     
    %  	$\model{rbf}{loc}\_64e4$  & 1.275& 1.307 %(0.000)
    %  	& 0.087 (0.000) & 10.9 (0.0)         
    %  	& 0.085 (0.000) & 10.7 (0.0) \\ %\hline
    %  	$\model{rbf}{loc}\_64e8$  & 1.259& 1.297 %(0.000)
    %  	& 0.094 (0.000) & 12.1 (0.0)         
    %  	& 0.096 (0.000) & 11.8 (0.0) \\ %\hline
    %  	$\model{rbf}{loc}\_64e16$  & 1.235& 1.286 %(0.000)
    %  	& 0.102 (0.000) & 13.4 (0.0)         
    %  	& 0.103 (0.000) & 13.0 (0.0) \\ %\hline
    %  	$\model{rbf}{loc}\_64e32$  & 1.230& 1.287 %(0.000)
    %  	& 0.103 (0.000) & 13.9 (0.0)         
    %  	& 0.103 (0.000) & 13.3 (0.0) \\ %\hline
    %  	$\model{rbf}{loc}\_64e64$  & 1.237& 1.283 %(0.000)
    %  	& 0.103 (0.000) & 13.5 (0.0)         
    %  	& 0.108 (0.000) & 14.3 (0.0) \\ %\hline

     	%\hline
%Place2Vec_center-10-64-0.5-mean-global-200-1000.0-rbf-64-16-1000000.0-relu-geometric-F-T--3-512-T-T-T-concat-leakyrelu-sigmoid-1-T-T-concat-leakyrelu-sigmoid-1-T-T-max-sigmoid-adam-0.001000-512
        % \_3h512e64
     	$\model{rbf}{loc}$ ($\sigma$=1k)  & 1.209& 1.279 %(0.000)
     	& 0.115 (0.001) & 15.2 (0.2)         
     	& 0.123 (0.001) & 16.8 (0.3) \\ %\hline
     	 \hline
     	$\model{grid}{loc}$   ($\lambda_{min}$=50) & 1.156 & 1.258 %(0.001)              
		& 0.128 (0.001) & 18.1 (0.3)       
		& 0.139 (0.001) & \textbf{20.0} (0.2) \\ %\hline
		$\model{hexa}{loc}$  ($\lambda_{min}$=50)  & 1.230 & 1.297 %(0.001)     
		& 0.107 (0.001) & 14.0 (0.2)        
		& 0.105 (0.001) & 14.5 (0.2) \\ % \hline
		$\model{theorydiag}{loc}$  ($\lambda_{min}$=50)  & 1.277 & 1.324 %(0.001)              
		& 0.094 (0.001) & 12.3 (0.3)         
		& 0.094 (0.002) & 11.2 (0.3)  \\  %\hline
		
% 		$\model{theory}{loc}$   &  & 1.295 %(0.001)                   
% 		& 0.099 (0.002) & 12.5 (0.4)        
% 		& 0.104(0.001) & 13.2 (0.4) \\ 
		
% 		$\model{theory}{loc}\_64e8$   &   1.312&1.331 %(0.001)
% 		& 0.084 (0.000) & 10.1 (0.0)        
% 		& 0.082(0.000) & 10.2 (0.0) \\ 
% 		$\model{theory}{loc}\_64e64$   &   1.260&1.312 %(0.001)                   
% 		& 0.090 (0.000) & 11.3 (0.0)        
% 		& 0.092(0.000) & 11.9 (0.0) \\ 
% 		 \hline
% % Place2Vec_center-10-64-0.5-mean-global-0-1000.0-theory-64-16-1000000.0-relu-geometric-T-T--1-512-T-T-T-concat-leakyrelu-sigmoid-1-T-T-concat-leakyrelu-sigmoid-1-T-T-max-sigmoid-adam-0.001000-512
% 		$16\_1m\_1\_1h512e64$   &   1.158&1.301 %(0.001)                   
% 		& 0.121 (0.000) & 15.8 (0.0)        
% 		& 0.117(0.000) & 16.2 (0.0) \\ 
% % Place2Vec_center/Place2Vec_center-10-64-0.5-mean-global-0-1000.0-theory-64-16-40000.0-50.0-relu-geometric-T-T--3-512-T-T-T-concat-leakyrelu-sigmoid-1-T-T-concat-leakyrelu-sigmoid-1-T-T-max-sigmoid-adam-0.001000-512.log
% 	$16\_40k\_50\_3h512e64$   &   1.114&1.256 %(0.001)      
% 		& 0.133 (0.000) & 17.9 (0.0)        
% 		& 0.137 (0.000) & 18.5 (0.0) \\ 
% % Place2Vec_center/Place2Vec_center-10-64-0.5-mean-global-0-1000.0-theory-64-16-100000.0-1000.0-relu-geometric-T-T--3-512-T-T-T-concat-leakyrelu-sigmoid-1-T-T-concat-leakyrelu-sigmoid-1-T-T-max-sigmoid-adam-0.001000-512.log
% 	$16\_100k\_1k\_3h512e64$   &   1.206&1.284 %(0.001)    
% 		& 0.120 (0.000) & 16.4 (0.0)        
% 		& 0.120 (0.000) & 16.6 (0.0) \\ 
% % Place2Vec_center/Place2Vec_center-10-64-0.5-mean-global-0-1000.0-theory-64-16-50000.0-500.0-relu-geometric-T-T--3-512-T-T-T-concat-leakyrelu-sigmoid-1-T-T-concat-leakyrelu-sigmoid-1-T-T-max-sigmoid-adam-0.001000-512.log
% 	$16\_50k\_500\_3h512e64$   &   1.185&1.265 %(0.001)    
% 		& 0.128 (0.000) & 17.3 (0.0)        
% 		& 0.129 (0.000) & 17.8 (0.0) \\ 
% \hline
%Place2Vec_center-10-64-0.5-mean-global-0-1000.0-theory-64-32-1000000.0-1000.0-relu-geometric-T-T--1-512-T-T-T-concat-leakyrelu-sigmoid-1-T-T-concat-leakyrelu-sigmoid-1-T-T-max-sigmoid-adam-0.001000-512.log
% 		$32\_1m\_1k\_2h512e64?$   &   1.081&1.245 %(0.001)  
% 		& 0.135 (0.000) & 19.0 (0.0)        
% 		& 0.143 (0.000) & 19.8 (0.0) \\ 
% Place2Vec_center-10-64-0.5-mean-global-0-1000.0-theory-64-32-1000000.0-1000.0-relu-geometric-T-T--3-512-T-T-T-concat-leakyrelu-sigmoid-1-T-T-concat-leakyrelu-sigmoid-1-T-T-max-sigmoid-adam-0.001000-512.log	
% 	$32\_1m\_1k\_3h512e64$   &   1.220&1.295 %(0.001)  
% 		& 0.110 (0.000) & 14.4 (0.0)        
% 		& 0.112 (0.000) & 14.6 (0.0) \\ 

		$theory$  ($\lambda_{min}$=1k)
		&   1.207 & 1.281 %(0.001)  
		& 0.123 (0.002) & 16.3 (0.5)        
		& 0.121 (0.001) & 16.2 (0.1) \\

%Place2Vec_center/Place2Vec_center-10-64-0.5-mean-global-0-1000.0-theory-64-32-50000.0-500.0-relu-geometric-T-T--3-512-T-T-T-concat-leakyrelu-sigmoid-1-T-T-concat-leakyrelu-sigmoid-1-T-T-max-sigmoid-adam-0.001000-512.log
%	$32\_50k\_500\_3h512e64$   
	$theory$  ($\lambda_{min}$=500) &   1.188&1.269 %(0.001)    
		& 0.132 (0.001) & 17.6 (0.3)        
		& 0.129 (0.001) & 17.7 (0.2) \\ 

% Place2Vec_center-10-64-0.5-mean-global-0-1000.0-theory-64-32-40000.0-50.0-relu-geometric-T-T--3-512-T-T-T-concat-leakyrelu-sigmoid-1-T-T-concat-leakyrelu-sigmoid-1-T-T-max-sigmoid-adam-0.001000-512.log
	%$32\_40k\_50\_3h512e64$  
	$theory$  ($\lambda_{min}$=50)
	&   1.098&1.249 %(0.001)  
		& \textbf{0.137} (0.002) & \textbf{19.4} (0.1)        
		& \textbf{0.144} (0.001)  & \textbf{20.0} (0.2) \\ 
%Place2Vec_center-10-64-0.5-mean-global-0-1000.0-theory-64-32-40000.0-50.0-relu-geometric-T-T--1-512-T-T-T-concat-leakyrelu-sigmoid-1-T-T-concat-leakyrelu-sigmoid-1-T-T-max-sigmoid-adam-0.001000-512.log
% 	$32\_40k\_50\_1h512e64$   &   1.081&1.244 %(0.001)  
% 		& 0.137 (0.000) & 19.4 (0.0)        
% 		& 0.144 (0.000) & 20.1 (0.0) \\ 
		\bottomrule
	\end{tabular}}	\vspace*{-0.25cm}
\end{table}


==> Location Encoding Paper - ICLR 2020/locmodel_stats.tex <==
\vsubsubsection{Multi-Scale Analysis of Location Modeling}
In order to show how our multi-scale location representation model will affect the prediction of POI types with different distribution patterns, we classify all 1,191 POI types into three groups based on radius $r$, which is derived from each POI types' renormalized Ripley's K curve (See Figure \ref{fig:ripley_log} for examples). 
It indicates the x axis value of the intersection between the curve and the line of $y = 3.0$. A lower $r$ indicates a more clustered distribution patterns. These three groups are listed below:
\begin{enumerate}
	\item Clustered ($r \leq 100m$): POI types with clustered distribution  patterns;
	\item Middle ($100m < r < 200m$): POI types with less extreme scales;
	\item Even ($r \geq 200m$): POI types with even distribution patterns.
\end{enumerate}



Table \ref{tab:locmol_stat} shows the performance ($MRR$) of $direct$, $tile$, $wrap$, $rbf$, and our $theory$ model on the test dataset of the location modeling task with respect to these three different POI distribution groups. The numbers in $()$ indicate the MRR difference betweeb a baseline and $theory$. \textit{\# POI} refers to total number of POI belong to each group\footnote{The reason why the sum of \textit{\# POI} of these three groups does not equal to the total number of POI is because one POI can have multiple types and they may belonging to different groups.}.
%
We can see that 
1) The two neural net approaches ($direct$ and $wrap$) have no scale related parameter and are not performing ideally across all scales, with $direct$ performs worse because of its simple single layer network.
2) The two approaches with built-in scale parameter ($tile$ and $rbf$) have to trade off the performance of different scales. Their best parameter settings lead to close performances to that of \modelname at the middle scale, while performing poorly in both clustered and regular groups.
%
These observation clearly shows that \textbf{all baselines can at most well handle distribution at one scale but show poor performances in other scales. In contrast, Space2Vec’s multi-scale representation can handle distributions at different scales.}




\begin{table}[t!]
	\caption{
	%The MRR comparison among $direct$, $tile$, $wrap$, $rbf$, and $theory$ model on location modeling task (See Section \ref{sec:loceval}). 
	    Comparing performances in different POI groups.
		We classify all 1,191 POI types into three groups based on the radius $r$ of their root types, where their renormalized Ripley's K curve (See Figure \ref{fig:ripley_log}) reach 3.0: 
		1) Clustered ($r \leq 100m$): POI types with clustered distribution patterns; 
		2) Middle ($100m < r < 200m$): POI types with unclear distribution patterns; 
		3) Even ($r \geq 200m$): POI types with even distribution patterns. The MRR of $wrap$ and $theory$ on those three groups are shown. 
		The numbers in $()$ indicate the difference between the MRR of a baseline model and the MRR of $theory$ with respect to a specific group.
		\textit{\#POI} refers to the total number of POIs belonging to each group.
		\textit{Root Types} indicates the root categories of those POI types belong to each group.
	}
	\label{tab:locmol_stat}
	\centering
	\small{
		\begin{tabular}{c|c|c|c}
			\toprule
			%	&    & 
			%\multicolumn{2}{c}
			\textbf{POI Groups} 
			&\textbf{Clustered}& \textbf{Middle} & \textbf{Even} \\% \hline
			 &  ($r \leq 100 m$)   &  ($100m < r < 200m$)   &  ($r \geq 200 m$)  \\ \hline
			$direct$   %& $MRR$
			& 0.080 (-0.047) & 0.108 (-0.030)    & 0.084 (-0.047)   \\
			$wrap$   %& $MRR$
			& 0.106 (-0.021) & 0.126 (-0.012)    & 0.122 (-0.009)   \\  \hline
			$tile$   %& $MRR$
			& 0.108 (-0.019) & 0.135 (-0.003)    & 0.111 (-0.020)   \\
			$rbf$   %& $MRR$
			& 0.112 (-0.015) & 0.136 (-0.002)    & 0.119 (-0.012)   \\ \hline
			$theory$% & $MRR$ 
			& 0.127 (-)  & 0.138  (-)   & 0.131 (-)   \\ \hline
			%	\multicolumn{2}{c|}	{$MRR_{theory} - MRR_{wrap}$} & 0.021  &0.012   & 0.009  \\ \hline
			%\multicolumn{2}{c|}
			{\# POI}       & 16,016  & 7,443   & 3,915   \\ \hline
			%\multicolumn{2}{c|}
			{Root Types}    & \begin{tabular}[c]{@{}l@{}}
			Restaurants; Shopping; Food; \\
			Nightlife;  Automotive; Active \\
			 Life; Arts \& Entertainment; \\
			Financial Services\end{tabular} 
			& 
			\begin{tabular}[c]{@{}l@{}}
			Beauty \& Spas; Health \& Medical;\\
			Local Services; Hotels \& Travel;\\
			Professional Services;\\
			Public Services  \& Government
			\end{tabular} 
			& 
			\begin{tabular}[c]{@{}l@{}}
			Home Services; \\
			Event Planning \\ 
			\& Services;\\
			 Pets; Education
			 \end{tabular} 
			 \\ \bottomrule
		\end{tabular}
	}	\vspace*{-0.25cm}
\end{table}

==> Location Encoding Paper - ICLR 2020/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Location Encoding Paper - ICLR 2020/method.tex <==
\vsection{Method} \label{sec:method}

We solve \textit{distributed representation of point-features in space} 
%unsupervised  inductive learning
(defined in Section \ref{sec:prob}) with  an encoder-decoder architecture:
\begin{enumerate}
%\item The encoder $\enc()$ with Paramater $\enctheta$ consists of two parts: 
%\item The \textbf{point space encoder} $\enc^{(x)}()$ with $\enctheta^{(x)}$ and point feature encoder $\enc^{(v)}()$ with $\enctheta^{(v)}$. 

\item Given a point $p_i=(\bx_i, \bv_i)$ a \textbf{point space encoder} $\enc^{(x)}()$ encodes location $\bx_i$ into a location embedding $\peemb{i} \in \Real^{\pedim}$ and a \textbf{point feature encoder} $\enc^{(v)}()$ encodes its feature into a feature embedding $\feemb{i} \in \Real^{\fedim}$.  
$\emb = [\peemb{i};\feemb{i}] \in \Real^{\embdim}$ is the full representation of point $p_i \in \mP$, where $\embdim = \pedim+\fedim$. 
$[;]$ represents vector concatenation. 
In contrast, geographic entities not in $\mP$ within the studied space can be represented by their location embedding $\peemb{j}$ since  
%it does not have feature $\bv_i$, or its feature 
its  $\bv_i$ is unknown.
\item 
%We propose two types of decoder: 
%The \textbf{location decoder} $\locdec()$ with $\locdectheta$ and spatial context decoder $\contdec()$ with $\contdectheta$.
We developed two types of decoders which can be used independently or jointly.
A \textbf{location decoder} $\locdec()$  reconstructs point feature embedding $\feemb{i}$ given location embedding $\peemb{i}$, and 
a \textbf{spatial context decoder} $\contdec()$ reconstructs the feature embedding $\feemb{i}$ of point $p_i$ based on the space  and feature embeddings $\{\emb_{i1},...,\emb_{ij},...,\emb_{i\neisize}\}$ of 
nearest neighboring points $\{p_{i1},...,p_{ij},...,p_{i\neisize}\}$, where $\neisize$  is a hyper-parameter. 
% for the number of neighbours considered.
\end{enumerate}

\input{encoder.tex}
\input{decoder.tex}

\vspace{-0.4cm}
\vsubsection{Unsupervised Training}  \label{sec:training}
The unsupervised learning task can simply be
%be setting up by 
%minimizing the loss shown in Equation \ref{equ:loss_gc}.
maximizing the log likelihood of observing the true point $p_i$ at position $\bx_i$  among all the points in $\mP$ 
%(See Equ. \ref{equ:loss_gc}).
\begin{align}
\label{equ:loss_gc}
\centering
\loss_\mP(\theta) = - %\dfrac{1}{|\mP|} 
\sum_{p_{i} \in \mP} \log  P(p_i|p_{i1},...,p_{ij},...,p_{i\neisize}) 
= - %\dfrac{1}{|\mP|} 
\sum_{p_{i} \in \mP} \log \dfrac{
	\exp(\feemb{i}^{T}\feemb{i}^{\prime})}{\sum_{p_{o} \in \mP} 
	\exp(\feemb{o}^{T}\feemb{i}^{\prime})}
\end{align}
Here only the feature embedding of $p_i$ is used (without location embedding) to prevent revealing the identities of the point candidates, and $\theta=[ \enctheta;  \dectheta]$

Negative sampling by \citet{mikolov2013distributed} can be used to improve the efficiency of training
%(See Equation \ref{equ:loss_neg_gc}).
\begin{align}
\label{equ:loss_neg_gc}
\centering
\loss_\mP'(\theta) &= - %\dfrac{1}{|\mP|} 
\sum_{p_{i} \in \mP} \Big( 
\log \sigma(\feemb{i}^{T}\feemb{i}^{\prime}) + 
\dfrac{1}{|\negsampi|}\sum_{p_{o} \in \negsampi} 
\log \sigma(-\feemb{o}^{T}\feemb{i}^{\prime})  
\Big)
\end{align}
Here $\negsampi \subseteq \mP$ is a set of 
% $\negsize$ 
sampled negative points for $p_{i}$  
($p_{i} \notin \negsampi$) and $\sigma(x) = 1/(1 + e^{-x})$.


==> Location Encoding Paper - ICLR 2020/problem.tex <==
\vsection{Problem Formulation}  \label{sec:prob}

%The problem of 
{\em Distributed representation of point-features in space} can be formulated as follows. 
Given a set of points $\mP=\{p_i\}$, i.e., Points of Interests (POIs), in $\spdim$-D space ($\spdim = 2,3$) 
%with $V$-dimension ML features 
define a function $f_{\mP,\theta}(\bx): \Real^{\spdim} \to \Real^\embdim$ ($\spdim \ll \embdim$), 
which is parameterized by $\theta$ and maps any coordinate $\bx$ in space to a vector representation of $\embdim$ dimension.
Each point (e.g., a restaurant) $p_i=(\bx_i, \bv_i)$ is associated with a location $\bx_i$ and  attributes $\bv_i$ (i.e., POI features such as type, name, capacity, etc.). 
The function $f_{\mP,\theta}(\bx)$ encodes the probability distribution of point features over space and can give a representation of any point in the space. Attributes (e.g. place types such as \textit{Museum}) and coordinate of point can be seen as analogies to words and word positions in %traditional 
commonly used
word embedding models. 
%to indicate the probability distribution of features at this specific location.


==> Location Encoding Paper - ICLR 2020/related.tex <==
\vspace{-0.2cm}
\section{Related Work}   \label{sec:related}
\vspace{-0.2cm}
% Previous work have explored ways to encode positions in space. PointNet \citep{qi2017pointnet} and PointNet++ \citep{qi2017pointnet++} directly encode point sets for supervised learning tasks such as 3D point cloud object classification and semantic segmentation. Recent work focus on directly encoding point sets in an unsupervised learning setting for  specific tasks. 
% For example, \citet{sauder2019context} propose unsupervised learning on raw 3D point cloud data by training a neural network to predict the spatial relationship between two point cloud segments. 
% %
% \mai{might need to rethink about this}
% Compared to this work which is designed for specific tasks and focusing on encoding position information of points, our proposed \modelname~{} model is a general unsupervised learning model (similar to BERT), and can be applied to various machine learning and spatial downstream tasks such as POI check-in prediction, geotagged image classification, and so on. 
% Moreover, \mai{while the input of PointNet is the entire point cloud, the input of \modelname~{} can be one single point and} \modelname~{} jointly considers the position and other attributes about a point-feature.


There has been theoretical research on neural network based path integration/spatial localization models and their relationships with grid cells. 
Both \citet{cueva2018emergence} and \citet{banino2018vector} showed that grid-like spatial response patterns emerge in trained networks for navigation tasks which demonstrate that grid cells are critical for vector-based navigation. 
Moreover, \citet{gao2018learning} propose a representational model for grid cells in navigation tasks which has good quality such as magnified local isometry. All these research is focusing on understanding the relationship between the grid-like spatial response patterns and navigation tasks from a theoretical perspective. In contrast, our goal focuses on utilizing these theoretical results
%conclusions about grid cells 
on real world data in geoinformatics.

Radial Basis Function (RBF) kernel is a well-established approach to generating learning friendly representation  
from points in space  
for machine learning 
algorithms such as SVM classification~\citep{baudat2011kernel} and regression~\citep{Bierens1994regression}.
However, the representation is example based
%almost always training data dependent 
-- i.e., the resultant model uses the positions of training examples as the centers of Gaussian kernel functions~\citep{mazya1996gaussian}.
In comparison, the grid cell based location encoding relies on sine and cosine functions, and  the resultant model is inductive and does not %need to 
store training examples.

Recently the computer vision community shows increasing interests in incorporating geographic information (e.g. coordinate encoding) into neural network architectures for multiple tasks such as image classification \citep{tang2015improving} and fine grained recognition \citep{berg2014birdsnap,chu2019geo,mac2019presence}. 
Both \citet{berg2014birdsnap} and \citet{tang2015improving} proposed to discretize the study area into regular grids. To model the geographical prior distribution of the image categories, the grid id is used for GPS encoding instead of the raw coordinates. However, choosing the correct discretization is challenging \citep{openshaw1984modifiable,fotheringham1991modifiable}, and incorrect choices can significantly affect the final performance \citep{moat2018refining,lechner2012investigating}. 
In addition, discretization does not scale well in terms of memory use. To overcome these difficulties, both \citet{chu2019geo} and \citet{mac2019presence} advocated the idea of inductive location encoders which directly encode coordinates into a location embedding. However, both of them directly feed the coordinates into a feed-forward neural network \citep{chu2019geo} or residual blocks \citep{mac2019presence} without any feature decomposition strategy. 
Our experiments show that this direct  encoding approach is insufficient to capture the spatial feature distribution and \modelname significantly outperforms them by integrating spatial representations of different scales.

